Automatic Database Configuration Debugging using Retrieval-Augmented Language Models

Database management system (DBMS) configuration debugging, e.g., diagnosing poorly configured DBMS knobs and generating troubleshooting recommendations, is crucial in optimizing DBMS performance. However, the configuration debugging process is tedious and, sometimes challenging, even for seasoned database administrators (DBAs) with sufficient experience in DBMS configurations and good understandings of the DBMS internals (e.g., MySQL or Oracle). To address this difficulty, we propose Andromeda, a framework that utilizes large language models (LLMs) to enable automatic DBMS configuration debugging. Andromeda serves as a natural surrogate of DBAs to answer a wide range of natural language (NL) questions on DBMS configuration issues, and to generate diagnostic suggestions to fix these issues. Nevertheless, directly prompting LLMs with these professional questions may result in overly generic and often unsatisfying answers. To this end, we propose a retrieval-augmented generation (RAG) strategy that effectively provides matched domain-specific contexts for the question from multiple sources. They come from related historical questions, troubleshooting manuals and DBMS telemetries, which significantly improve the performance of configuration debugging. To support the RAG strategy, we develop a document retrieval mechanism addressing heterogeneous documents and design an effective method for telemetry analysis. Extensive experiments on real-world DBMS configuration debugging datasets show that Andromeda significantly outperforms existing solutions.

==> algs/metric_analysis.tex <==
\begin{small}

\begin{algorithm}[t!]
	\caption{Metric analysis} 
        \label{alg:metric_analysis}
        \KwIn{Issue $q_{query}$, Telemetry $T_S$ with metric set $S$}
        \KwOut{Text description $P$}

        Initialize the maximum iteration time $N$.

        Initialize the number of descriptions $K$.
        
        Initialize anomalous metric deviation set $\mathbb{A}$.

        Initialize description set $\mathbb{P}$.
        
        \BlankLine
        \tcp{Anomalous metric deviation detection}
        \For{each metric temporal data $T_{s_i} \in T_S$}{
            \For{each $k \in 1, 2, ..., N$}{
                $Seasonal_{s_{i}}, Trend_{s_{i}}, \epsilon_{s_{i}} = STL(T_{s_{i}})$

                
                Calculate the critical value  $\lambda_k$ as threshold using Equation~\ref{equ:lambda}

                \For{each value $t_j$ on timestamp $j$ in $T_{s_i}$}{
                    Calculate the deviation score $C_{t_{j}}$ using Equation~\ref{equ:deviation}.  
                }

               $C_{max}, j_{max} = \max_{t_j \in T_{s_i}} C_{t_{j}}$
               
               \If{$C_{max} > \lambda_k$}{
               Add $(s_i, j_{max}, t_{j_{max}}, T_{s_i})$ to $\mathbb{A}$.

               Drop $t_{j_{max}}$ from $T_{s_i}$.
               }
            }
        }

        \tcp{Deviation description and selection.}
        
        
        
        \For{each $(s_i, j, t_{j}, T_{s_i}) \in \mathbb{A}$ }{
            $p_{s_i}, \mathbb{k}_{s_i} = Generate\_text(s_i, j, t_{j}, T_{s_i})$

            Add $(p_{s_i}, \mathbb{k}_{s_i})$ to $\mathbb{P}$.
        }
        
        $\mathbb{P} = topKSemanticSimilarity(q_{query}, \mathbb{P}, K)$

        $P = concatenate(\mathbb{P})$

        
\end{algorithm}

\end{small}

==> response/revision-letter.tex <==
%!TEX root = ../main.tex
\subsection*{Dear SIGMOD Meta-Reviewer and Reviewers,}

\noindent 
Thank you for your encouraging comments, based on which we have made a substantial revision, with the updated contents highlighted in \revised{blue}.
Below, we first summarize the \textbf{main changes} in our revision, followed by \textbf{detailed responses} to each reviewer.

%\section*{Revision Plan}


%
%We will conduct case studies, where we sample some user questions that Andromeda successfully addressed, and some cases that Andromeda failed, analyzing how Andromeda works and the room of improvement.



%We have conducted sensitivity experiments of different queries' knob type and queries' knob frequency in Figure 7, Figure 8 and Figure 9. If more sensitivity experiments are needed, we can add them when revising the paper. Moreover, we will conduct case studies to show which queries are successfully solved and which are failed with analyzing the reasons.


\stitle{M1 [More Baselines]}: We have added more baselines. 
(1) For PLMs, we augment the training data for the PLM using our proposed techniques in {Section~\ref{sec:da}}, and introduce a new baseline \emph{DA + PLM}.

(2) For LLMs, we add the following new baselines. 
\begin{itemize}
\item We replace GPT with other LLMs, \ie using Qwen2 and Llama-3 at two different scale levels (less than 10B and larger tnan 70B) for the new baselines, \emph{Qwen}, \emph{Llama-3}, \emph{Qwen (all knobs)}, \emph{Llama-3 (all knobs)}, \emph{\sys-Qwen}, and \emph{\sys-Llama-3}. 
\item We consider \emph{Prompt Engineering} baselines, such as chain-of-thought and task decomposition. 
\item We consider an \emph{SFT} baseline that fine-tunes GPT-3.5 using our training data. 
\end{itemize}
%
We provide details of the above baselines in \textbf{Section~\ref{sec:exp-setup}}, report the results in \textbf{Table~\ref{tab:overall}} and analyze the results \textbf{Exp-1 in Section~\ref{sec:exp-overall}}.
The results show that \sys outperforms all the baselines.

%
%For PLM, we will use the same training method of PLM with augmented training data (\textbf{DA + PLM}). For LLM, we will add the following baselines.
% \textbf{(1) More models:} add more large language models to replace GPT in our existing experiments. Specifically, we use Qwen, Llama-3 to replace GPT with the following baselines - \textbf{Qwen, Llama-3, Qwen (all knobs), Llama-3 (all knobs)}. Moreover, we also replace GPT in \sys as \sys-Qwen, \sys-llama-3. \textbf{(2) Varying prompts}: add more prompt engineers (CoT, task decompose). \textbf{(3) Fine-tuning}: fine-tune GPT 3.5 using the training data.
 
\stitle{M2 [Larger Datasets]}: We have increased the number of test questions to 100 in the Runnable setting, as shown in \textbf{Table~\ref{tab:dataset}}. 

However, it is challenging to expand the datasets in the NL setting, as we have already gathered nearly all knob-configuration-related questions for MySQL and PostgreSQL from StackOverflow and the MySQL forum.

%, it is hard to scale. For the runnable setting, we will add more questions to around 100.

\stitle{M3 [New Experiments: End-to-end Time Reduction]}:
We have added a new experiment to evaluate whether \sys effectively reduces the end-to-end time.
% in the Runnable setting.
% (i.e., the operational burden) for DBAs during database configuration debugging. 
%
Specifically, we employ experienced DBAs and provide them with historical questions, database manuals, and telemetry data. We then consider three strategies: (1) \term{using manuals}: DBAs manually search DBMS manuals to provide diagnostic suggestions for tuning knobs; (2) \term{using search engines}: DBAs use search engine to provide diagnostic suggestions for tuning knobs; (3) \term{using \sys}: DBAs follow \sys's recommendations to address the issues. We compare the average time taken by the DBAs to troubleshoot configuration issues, thereby demonstrating the effectiveness of \sys. 

The results are reported in \textbf{Table~\ref{tab:user_study}}, and the analysis is presented in \textbf{Exp-7 in Section~\ref{sec:exp-eff}}. We find that \sys can effectively reduce the end-to-end time (\ie the operational burden) for DBAs, while still preserving higher SuccessRate. 



% 
% We will add a user study to evaluate \sys's time cost. Specifically, we will first invite two experienced DBAs to manually solve the problems with provided historical questions, database manuals and telemetries and record the time cost. Second, we will ask two other experts with the same ability to solve the problem using \sys and record the time cost. Finally, we will compare these two records to show how \sys works.

\stitle{M4 [New Experiments: Sensitivity to Noise Sources]}: 
We have conducted experiments to examine whether inaccuracies in the retrieval sources (\eg, historical questions, troubleshooting manuals and telemetry data) impact the overall performance of \sys. We manually inject noise into these sources by replacing the ground-truth labels in historical questions or database manuals with incorrect ones at a various probability (e.g., 10\%). 

The results are reported in \textbf{Exp-4 in Section~\ref{sec:exp-doc}}, which show that inaccuracies in the retrieval sources impact the performance, highlighting the importance of the quality of retrieval sources.



% We then evaluate \sys's performance on both retrieval effectiveness (e.g., recall) and overall performance.
%We find that inaccuracies in the retrieval sources impact the overall performance of \sys.

%\sibei{need updated}. We use the completeness of the included knobs to indicate the quality of the source. We will add a sensitivity experiment to reduce the knobs contained in the source to evaluate the impact of different source quality on \sys performance.

\stitle{M5 [New Experiments: Scalability of Telemetry Data Analysis]}: 
We have added new experiments to examine the scalability of our approach for detecting relevant telemetry data. Specifically, we vary the timestamp interval of each metric and the number of metrics, and report the time required for telemetry data analysis. 

As reported in \textbf{Exp-8 in Section~\ref{sec:exp-eff}}, \sys performs well in terms of scalability for telemetry data analysis.

%We find that the scale of telemetry data does not significantly affect the time of telemetry analysis, which can be kept
%within a few seconds.
%
%
%We will analyze different scales of telemetry by gradually reducing the metric types and timestamps and evaluate their results.

% \stitle{M7 [New Experiments: Effect of Additional Contextual Information]}: 
% We have conducted new experiments to investigate the impact of providing additional contextual information to prompt the LLM, specifically focusing on \emph{DB statistics from the tables}. We utilize the table names, the number of tuples, column names, and column data types as the DB statistics. We added this information to origin \sys and use GPT 3.5 to evaluate it. The accuracy of dataset ``MySQL Run'' in runnalbe setting is $0.61$, which is lower than \sys (0.79). We infer that the current three sources (historical questions, DBMS manuals and telemetry) are sufficient, and providing more information for the LLM may actually affect its predictions.

% We then evaluate whether this information is beneficial and analyze the underlying reasons.

\stitle{M6 [New Experiments: Cost Efficiency]}: 
We have reported the cost efficiency, which is the average cost of calling LLMs for each NL debugging question in \textbf{Exp-9 in Section~\ref{sec:exp-eff}}. We find that \sys has good performance on cost efficiency.

%
%We will evaluate the overall quality after adding DB statistics from the tables. In particular, we use a template to transfer DB statistics to a text description. Then we add it to \sys's prompt (containing historical questions, manuals and telemetries) and evaluate the reasoning results, comparing it with original \sys.

\stitle{M7 [More In-Depth Experimental Analysis]}:

(1) We have provided more in-depth analysis by categorizing questions by their types in \textbf{Exp-5 in Section~\ref{sec:exp-tel}} for evaluating telemetry data analysis, and by their frequencies in \textbf{Exp-3 in Section~\ref{sec:exp-doc}} for evaluating document retrieval.
%

(2) We have reported precision and recall  in \textbf{Table~\ref{tab:overall}} to make the comparison more comprehensive in \textbf{Exp-1 in Section~\ref{sec:exp-overall}}.
%

(3) We have further discussed the coverage of the evaluation datasets, with a specific focus on the percentage of MySQL/PostgreSQL knobs covered in the documentation, manuals, and test datasets in \textbf{Table~\ref{tab:dataset} in Section~\ref{sec:exp-setup}}.


%\textbf{(1) Adding recall / precision results}- We will add recall /precision scores in the NL setting for the overall evaluation. \textbf{(2) Adding statistics information} -  We will add more statistics including knob coverage in training questions, historical questions, manuals, and test questions.

\stitle{M8 [More Clarifications on Experimental Setup]}: 
We have provided more clarifications on the experimental setup in \textbf{Section~\ref{sec:exp-setup}}, with a particular focus on explaining that the training labels can be automatically annotated.
%in Section~\ref{sec:exp-setup}. 
%For the original training data, we use regular expressions to extract relevant knobs from accepted answers or comments on questions from StackOverflow or the MySQL Forum. For the augmented training data, we generate questions based on a knob's manual, with the knob serving as the label corresponding to the questions.
%To validate the labeling quality, we have randomly sampled some training and testing cases for manual verification, which have confirmed that our automatic labeling method is accurate.


\stitle{M9 [Additional Related Work]}: 
We have revised the Related Work in \textbf{Section~\ref{subsec:rw}}
to include a detailed discussion of traditional IR techniques to analyze the unique challenge of IR approaches.
%We will also analyze that, compared to traditional IR approaches, the unique challenge here lies in retrieving documents from multiple sources, such as historical questions and DBMS manuals, where the semantics of documents from different sources may be heterogeneous. For instance, in Figure 2, historical questions typically describe ``what is wrong'' (\eg ``\emph{It takes over 15 minutes\ldots}''), while DBMS manuals focus on ``how to fix it'' (\eg ``\emph{turn off autocommit mode}''). Moreover, it is hard for existing IR techniques to analyze telemetry data in the DBMS debugging scenarios.

%
%Generally speaking, existing IR algorithms aim to match queries and documents. There are three challenges in the DBMS configuration scenario. 
%    (i) The semantics of documents from different sources may be heterogeneous. For example, historical questions typically describe ``what is wrong'', while DBMS manuals focus on ``How to fix it''. 
 %   (ii) For existing IR algorithms, there is a lack of sufficient high-quality training data for DBMS configuration problem. 
 %   (iii) It is hard for existing IR algorithms to analyze telemetry data. In general, DBMS configuration requires reasoning and cannot be solved by direct text matching.


\stitle{M10 [Clarifications on Design Choices]}: 
We further clarify our design choices, particularly focusing on the following aspects.

% We have revised \textbf{Section~\ref{sec:framework}} to better clarify our design choices, specifically a particular focus on the following aspects.

% (1) There could be multiple ways, such as different tuning knobs, to fix the same issue. \sys uses an LLM to reason about the various tuning knobs and select the most appropriate set. 
% Specifically, \sys generates a prompt that includes all the retrieved data and then calls the LLM to recommend the configurations.

% (2) We also justify why using LLMs to predict knob value makes sense. There are two main reasons in Section~\ref{fig:framework}. Moreover, we agree that we need more techniques to optimize the configuration value reasoning using LLM such as dealing with numeric value more smartly. We have explained it in our future work (Section~\ref{sec:conclusion}). 


(1) There could be multiple ways, such as different tuning knobs, to fix the same issue. \sys uses an LLM to reason about the various tuning knobs and select the most appropriate set. 
Specifically, \sys generates a prompt that includes all the retrieved data and then calls the LLM to recommend the configurations. It is clarified in \textbf{Section~\ref{sec:framework} Step 3: Configuration Reasoning.} 

(2) We justify two main reasons of using LLMs to predict knob values in \textbf{Section~\ref{sec:framework} Step 3: Configuration Reasoning}. 

(3) We agree that we need more techniques to optimize the configuration value reasoning using LLM such as dealing with numeric value more smartly. We have explained it in our future work (see \textbf{Section~\ref{sec:conclusion}}). 


%
%because LLM can not only utilize the in-context knowledge with RAG but also some database related knowledge in the pre-training / fine-tuning process, which is helpful for knob value decisions.
%Clarification on reasoning configuration value
%There are two reasons why LLMs work. 
%    (i) Using RAG, LLM can obtain knowledge about the knobs. For example, LLM can set autocommit=0 with manual "when importing data into InnoDB, turn off autocommit mode, because…", and it can set $innodb\_log\_file\_size=256M$ if the similar question sets the same value. 
%    (ii) LLMs may learn some common settings in pre-training or finetuning phase. Moreover, we agree that we need more techniques to optimize the configuration value reasoning using LLM such as dealing numeric value more smartly. We will explain it in our future work. 

\stitle{M11 [Discussion on Generalizability]}:
We have added a discussion in \textbf{Section~\ref{sec:framework}} to justify that \sys can be easily generalized to other DBMSes.
%We will add a discussion in Section 3 to justify that \sys can be easily generalized to other DBMSes, as the algorithms for training data generation, model training, and evaluation are adaptable to new DBMSes. Specifically, when applying \sys to a new DBMS, all that is required is the specification of the knobs and the manuals of the DBMS. \sys can then use these inputs to automatically generate augmented data and train a new model during the offline stage, while supporting evaluation on the DBMS in the online stage.
 % M8 - more detailed experiment analysis
 % (1) Adding recall / precision results
 % (2) Adding statistics information

 % M9 - Including IR literature in related works.
% M10 - clarification on reasoning configuration value
% M11 - clarification on automating training label

 \stitle{M12 [Case Studies]}: We have added \emph{good cases} to demonstrate the user questions that \sys successfully addressed, and the \emph{failure cases} where \sys does not perform well, followed by an analysis of limitations of \sys and how \sys can be further improved.

Due to space limit, we have to put the case studies in \textbf{Appendix~\ref{sec:case_study}} in our technical report\revised{~\cite{techreport}}.
%which is also submitted as supplementary materials. 

% \stitle{M2 [New Experiments]}: We will conduct new experiments:
% \begin{enumerate}
%     \item
%     \textbf{More baselines}: For PLM, we will use the same training method of PLM with augmented training data (\textbf{DA + PLM}). For LLM, we will add the following baselines.
%  \textbf{(a) More models:} add more large language models to replace GPT in our existing experiments. Specifically, we use Qwen, Llama-3 to replace GPT with the following baselines - \textbf{Qwen, Llama-3, Qwen (all knobs), Llama-3 (all knobs)}. Moreover, we also replace GPT in \sys as \sys-Qwen, \sys-llama-3. 
% \textbf{(b) Varying prompts}: add more prompt engineers (CoT, task decompose). 
% \textbf{(c) Fine-tuning}: fine-tune GPT 3.5 using the training data.
%  \item \textbf{More retrieval sources}: We will evaluate the overall quality after adding DB statistics from the tables. In particular, we use a template to transfer DB statistics to a text description. Then we add it to \sys's prompt (containing historical questions, manuals and telemetries) and evaluate the reasoning results, comparing it with original \sys.
%  \item \textbf{Time cost quantification}: We will add a user study to evaluate \sys's time cost. Specifically, we will first invite two experienced DBAs to manually solve the problems with provided historical questions, database manuals and telemetries and record the time cost. Second, we will ask two other experts with the same ability to solve the problem using \sys and record the time cost. Finally, we will compare these two records to show how \sys works.

%  \item \textbf{Adding recall / precision results}: We will add recall /precision scores in the NL setting for the overall evaluation.
% \item \textbf{Sensitivity of source quality}: We use the completeness of the included knobs to indicate the quality of the source. We will add a sensitivity experiment to reduce the knobs contained in the source to evaluate the impact of different source quality on \sys performance.

% \item \textbf{Sensitivity of telemetry scale}: We will analyze different scales of telemetry by gradually reducing the metric types and timestamps and evaluate their results.

% \item \textbf{Adding statistics}: We will add more statistics including knob coverage in training questions, historical questions, manuals, and test questions.

% \item \textbf{Dataset}: For the NL setting, we have obtained almost all knob configuration related questions in StackOverflow dataset and MySQL community, it is hard to scale. For the runnable setting, we will add more questions to around 100.

% \end{enumerate}

% \stitle{M3 [Clarifications]}: We will make the following clarifications:

% \begin{enumerate}
%     \item \textbf{Compared with IR literature}: Generally speaking, existing IR algorithms aim to match queries and documents. There are three challenges in the DBMS configuration scenario. 
%     (i) The semantics of documents from different sources may be heterogeneous. For example, historical questions typically describe ``what is wrong'', while DBMS manuals focus on ``How to fix it''. 
%     (ii) For existing IR algorithms, there is a lack of sufficient high-quality training data for DBMS configuration problem. 
%     (iii) It is hard for existing IR algorithms to analyze telemetry data. In general, DBMS configuration requires reasoning and cannot be solved by direct text matching.

%     \item \textbf{Reasoning configuration value}: There are two reasons why LLMs work. 
%     (i) Using RAG, LLM can obtain knowledge about the knobs. For example, LLM can set autocommit=0 with manual "when importing data into InnoDB, turn off autocommit mode, because…", and it can set $innodb\_log\_file\_size=256M$ if the similar question sets the same value. 
%     (ii) LLMs may learn some common settings in pre-training or finetuning phase. Moreover, we agree that we need more techniques to optimize the configuration value reasoning using LLM such as dealing numeric value more smartly. We will explain it in our future work. 

%     \item \textbf{Automating training label}:  The training label can be automated annotated. For the real training data, we use regular expressions to match related knobs from accepted answers or comments of questions. For augmented training data, we generate questions based on a knob’s manual, and this knob is the label corresponding to the questions. We will explain it more clearly in our paper.
% \end{enumerate}

\section*{Responses to Reviewer \#1}

\begin{shaded}
\noindent\textit{\textbf{R1O1}: Experimental eval should include a few other baselines that use LLMs for solving the same problem\ldots}
\end{shaded}

\noindent\textbf{RESPONSE}: 
Thanks for the suggestion. To the best of our knowledge, we are the first to develop an LLM-based DBMS diagnosis system designed to accept NL questions on DBMS configuration issues and recommend specific configurations to address the issues. 
In response to your concern, we have added more baselines by substituting GPT with other LLMs, \eg Qwen and Llama-3. Please refer to \textbf{M1} in our revision plan for details.

\begin{shaded}
\noindent\textit{\textbf{R1O2}: There seems to be a lot of human effort required in collecting ground labels for training and evaluation (including confirmation by experts). Human in the loop in ML requires non-trivial amount of time and dollar cost. More discussion is needed.}
\end{shaded}

\noindent\textbf{RESPONSE}: 
We apologize for the confusion. \sys does not require significant human effort to collect ground truth labels for training and evaluation, thanks to its automated labeling process. We have revised the experimental setup (\textbf{Section~\ref{sec:exp-setup}}) for greater clarity. Please refer to \textbf{M8} for further details.


\begin{shaded}
\noindent\textit{\textbf{R1O3}: Related to the above point, the goal of \sys is to reduce the time it takes to manually arrive at a solution by expert DBAs. How could the paper quantify this claim?}
\end{shaded}

\noindent\textbf{RESPONSE}: We added new experiments to evaluate {\bf end-to-end time} of DBAs to solve issues with / without \sys, to qualify how \sys reduces the time. Please see \textbf{M3} for details.
 
\begin{shaded}
\noindent\textit{\textbf{R1O4}: the overall F-1 scores from Table 2 are still not very high for \sys. There seems to be a lot of room for improvement.}
\end{shaded}

\noindent\textbf{RESPONSE}: 
First, we would like to explain why the overall F-1 scores for \sys, as shown in Table 2, are not particularly high. As discussed in \textbf{Section~\ref{sec:exp-setup}}, the evaluation in the NL setting requires that \sys's output knobs strictly match the automatically labeled answers, while disregarding other potentially valid knobs. 
This constraint can lead to an underestimation of the F1 score, which is why we proposed the Runnable setting. In this setting, DBMS experts assess whether the recommended configurations resolve the issues. As shown in \textbf{Table~\ref{tab:overall}}, \sys achieves a SuccessRate of over 0.7.

We also acknowledge that ``there seems to be a lot of room for improvement''. We encourage a call to action to significantly advance this core database problem. To support this effort, we have conducted a thorough analysis of the less favorable cases produced by \sys. Please refer to {\bf M12} for further details.


%In the NL setting, it requires that the output knobs must be strictly the same as the answer, while ignoring some other knobs that may be valid. This is the reason for the low F1-score and why we propose the Runnable setting. To show this, we will add case studies for bad cases. Please see \textbf{M1} for details. We agree that ``there seems to be a lot of room for improvement'' -- we really hope for a call-to-arms 
%to significantly push this core database problem.

\begin{shaded}
\noindent\textit{\textbf{R1O5}: What was the actual prompt submitted to the LLM? It wasn't presented in the main body of the paper.}
\end{shaded}

\noindent\textbf{RESPONSE}: 
Please refer to \textbf{Figure~\ref{fig:running-example}(b)} as an illustrative prompt submitted to the LLM. To make it clearer, we have added more real prompts in experiments in our case studies (see \textbf{M12}). Moreover, we have already included all the prompts in our experiments in the repo: 
\url{https://anonymous.4open.science/r/Andromeda-D150/}

\begin{shaded}
\noindent\textit{\textbf{R1O6}: it would also be particularly insightful to discuss some loss cases for \sys for which it does not do well and how \sys could be improved to address those loses?}
\end{shaded}

\noindent\textbf{RESPONSE}: We have included a detailed analysis of the bad cases to highlight the limitations of \sys and discuss potential improvements. Please refer to \textbf{M12} for more details.

\begin{shaded}
\noindent\textit{\textbf{R1O7}: How generalizable is \sys to other DBMSes? Would it required training data generation, model training, and evaluation for each DBMS?}
\end{shaded}

\noindent\textbf{RESPONSE}: 
\sys can be generalized to other DBMSes. Please see \textbf{M11} for more details. 
% it needs to regenerate augmented data and retrain a new model in the offline stage because different DBMSs contain different knobs and manuals. Nevertheless, the algorithms for DA and training can be generalized.

\begin{shaded}
\noindent\textit{\textbf{R1O8}: The paper talks about the time efficiency of \sys but a discussion on the cost efficiency is missing.}
\end{shaded}

\noindent\textbf{RESPONSE}: As suggested, we have reported the cost efficiency, which is the average cost of calling LLMs for each NL debugging question $q$. Please see \textbf{M6} for more details. 

%Thanks for the suggestion. To calculate the cost of each query, we have calculated the average cost of prompt and response respectively and we add the prompt cost and response cost as the cost efficiency. In detail, 
%\begin{itemize}
%    \item GPT-3.5 costs $0.0017$\$ / query. 
%    \item GPT-4 costs $0.053$\$ / query. 
%    \item GPT-3.5 (all knobs) costs $0.012$\$ / query. 
%    \item GPT-4 (all knobs) costs $0.039$\$ / query.
%    \item \sys-3.5 costs $0.006$\$ / query.
%    \item \sys 4 costs $0.022$\$ / query.
%\end{itemize}

%We will add a more detailed report on the cost efficiency in experiments.

\stitle{Minor Remarks:}

\begin{shaded}
\noindent\textit{\textbf{R1C1}: It appears all telemetry data is always analyzed in real-time? There seems to be a lot of room for optimization here. %Please comment.
}
\end{shaded}

\noindent\textbf{RESPONSE}: 
Yes, the telemetry data is analyzed in real-time. We have conducted a latency analysis, as reported in \textbf{Table~\ref{tab:latency}}. The result shows that the time used for telemetry analysis is 2.85 seconds, which we believe is acceptable for users. 
However, we agree that there is room for optimization, such as filtering out unnecessary telemetry data. We will address this in future work.

%Yes, the telemetry data is analyzed in real-time. Actually, we have conducted the latency analysis in Table 8. The time consumption is in seconds, which we think is acceptable to users. In addition, we agree that there exists room for optimization, such as filtering useless telemetry. We will add it in our future work.

\begin{shaded}
\noindent\textit{\textbf{R1C2}: How does \sys (and related approaches) deal with cases where a small variation of a question compared to a historical question leads to a very different solution?}
\end{shaded}

\noindent\textbf{RESPONSE}: 
\sys deals with these cases by matching domain-specific contexts from other sources, including troubleshooting manuals and DBMS telemetry data. This is one of the key reasons we use multiple sources in our RAG approach. Specifically, when relying solely on historical questions is not sufficient, prioritizing relevant manuals or telemetry data over potentially confusing historical questions can provide more accurate solutions.


%\sys addresses these cases by matching domain-specific contexts for the question from other sources, including troubleshooting manuals and DBMS telemetries. Actually, this is the key reason that motivates us to use multiple sources for RAG. Specifically, when using single historical questions as sources is not helpful, ranking the helpful manuals/telemetries before this confusing historical question may help.

%For those cases where a small variation of a question compared to a historical question leads to a very different solution, using single historical questions as sources is not helpful. To deal with it, \sys uses multiple sources for RAG, for example, ranking the helpful manuals before this confusing historical question can help.

\begin{shaded}
\noindent\textit{\textbf{R1C3}: there could be multiple ways to fix the same issue? It's unclear how \sys and related approaches are reasoning about and ranking between different tuning knobs?}
\end{shaded}

\noindent\textbf{RESPONSE}: Yes, there could be multiple ways, such as different tuning knobs, to fix the same issue, as illustrated in \textbf{Figure~\ref{fig:running-example}(b)}. \sys uses an LLM to reason about the various tuning knobs and selects the most appropriate set. Please see \textbf{M10} for details. 

%Specifically, as discussed in \emph{Step 3} of the online stage in Section 3, \sys generates a prompt that includes all the retrieved data and then calls the LLM to recommend the configurations, i.e., the tuning knobs, to address the issue. We will revise Section 3 to clarify this further.

%
%Yes, there could exist multiple ways, \ie tuning knobs, to fix the same issue, as shown in Figure 2(b). \sys relies on an LLM to reason about between different tuning knobs and identify an appropriate set of knobs. Specifically, as discussed in \emph{Step 3} in the online stage of Section 3, \sys generates an prompt by including all the retrieved data and calls an LLM to generate the configuration recommendations, \ie tuning knobs, to fix the issue. We will revise Section 3 to make it clearer. 

%
%For the reasoning of \sys, it outputs the most related knobs using LLM to select knobs from candidate knobs in multi-sources as the top-1 result for the query. 

\begin{shaded}
\noindent\textit{\textbf{R1C4}: %In Sec 4.3, it's unclear by 
	why manual-manual samples are prioritized over others?}
\end{shaded}

\noindent\textbf{RESPONSE}: 
We conducted an experiment to evaluate different prioritization strategies, and the results show that prioritizing manual-manual training samples yields the best performance. The primary reason is that aligning manual-manual samples is ``easier'' than aligning question-question or manual-question samples due to the formality and consistency of manuals. By training our Alignment component on these easier cases first, we ensure it is well-prepared before gradually improving it on more challenging cases.
%
%We conducted an empirical evaluation of various configurations and found that prioritizing manual-manual samples yields the best quality. Our analysis suggests that optimizing models individually first benefits joint training. Specifically, optimizing the manual embedding model with manual-manual samples and the question embedding model with question-question samples leads to better performance when training multiple models using question-manual samples.
% Manual-manual samples are prioritized over others, because training manual-manual samples is the basis for training question-manual / manual-question samples. Given a question, the target of training manual-manual samples is to correctly represent manuals in hidden space to deal with multi-source heterogeneity. And after manuals currently embedded, \sys should learn to adjust question and manual embeddings based on the trained manual embeddings. 


\begin{shaded}
\noindent\textit{\textbf{R1C5}: %The document embeddings are stored in a vector DB. May be some quick mention of 
	what kind of vector DB and what kind of and size of indexes are needed to meet the runtime SLA of \sys?}
\end{shaded}

\noindent\textbf{RESPONSE}: We use Meta Faiss as our vector database to index the embeddings of historical questions and manuals. In the current implementation of \sys, we have indexed 5,138 vectors for MySQL and 1,158 vectors for PostgreSQL, with each vector having a dimension of 768. We have provide further clarification on this further in \textbf{Section~\ref{sec:exp-setup}}.

\begin{shaded}
\noindent\textit{\textbf{R1C6}: Analyzing a large amount of telemetry data and zooming in on the sections that might be correlated with the issue being debugged does not seem to be a new challenge and there may already be existing approaches.}
\end{shaded}

\noindent\textbf{RESPONSE}: 
There are two key challenges that distinguish our work. First, detecting anomalous telemetry data from vast amounts of time-series information is particularly difficult due to the influence of seasonality and trends, which can obscure what is truly anomalous. Second, existing approaches do not address the semantic correlation between natural language queries and telemetry data, which is an essential aspect of our solution.
% There are two new challenges: The first challenge is detecting anomalous telemetries from a huge amount of time-series data, as it is not easy to identify what is anomalous with the influence of sessonal and trand. Secondly, existing works do not consider the sematic correlation of the NL query and telemetries.
% We are the first to deal with user database diagnosis text questions using telemetry data. In detail, existing works analyze telemetry through only one aspect (such as the d-bot use rule to detect anomaly in telemetry). In contrast, our work comprehensively analyzes telemetry from multiple aspects that are anomalies in time series data of metric, the correlation of query and metrics with the description of metrics in manual. 

%
%\begin{shaded}
%\noindent\textit{\textbf{Required Changes}: O1, O2, O4, O6, %O8 (and addressing minor comments)}
%\end{shaded}
%
%\noindent\textbf{RESPONSE}: We have addressed all concerns. %Please see our responses mentioned above.
\vspace{-1em}
\section*{Responses to Reviewer \#2}

\begin{shaded}
\noindent\textit{\textbf{R2O1}: The experimental setup and findings lack sufficient details \ldots
	 %to aid understanding. For example, 
	 (1) the paper should explore which types of queries LLMs perform well on, where RAG helps, and whether historical queries can be categorized by type and frequency. It should also examine how the system performs for queries with less frequent questions. 
	 %
	 (2)Including results on precision and recall in Table 2 would also help.}
\end{shaded}

\noindent\textbf{RESPONSE}: 
%Thank you for the suggestion. 
We have revised the paper by providing more details about experimental setup and findings.

(1) We have already categorized queries by considering the frequency and types of their ground-truth labels (i.e., the tuning knobs) in \textbf{Section~\ref{sec:exp-doc}} and \textbf{Section~\ref{sec:exp-tel}}. Specifically, as shown in \textbf{Figures~\ref{fig:freq_retrieval} and \ref{fig:freq_reasoning}}, we classify queries into high-, medium-, and low-frequency categories. We also explore the questions raised by the reviewer. For instance, in most cases, LLMs perform better on high-frequency queries compared with medium- and low-frequency ones, while RAG consistently improves performance across all frequency levels. We examine \sys's performance on less frequent queries. In \textbf{Figure~\ref{fig:type}}, we further categorize queries by the type of their corresponding knobs (i.e., numerical, categorical, and boolean). Our findings show that \sys achieves better performance on numerical and boolean queries compared to categorical ones. 

(2) As suggested, we have included precision and recall results in \textbf{Table~\ref{tab:overall}} to make the comparison more comprehensive.

We have revised the paper to include detailed explanations of these experimental findings, as indicated in \textbf{M7}. 

%Thanks for the suggestions. As discussed in \textbf{M1}, We have conducted sensitivity experiments of the type of knob in different queries and the frequency of the knob in the queries in Figure 7, Figure 8 and Figure 9. If more sensitivity experiments are needed, we can add them when revising the paper. Moreover, we will conduct case studies (see \textbf{M1})to show which queries are successfully solved and which are failed in analyzing the reasons. And we will add recall / precision in Table 2.

\begin{shaded}
\noindent\textit{\textbf{R2O2}: Traditional IR techniques have long addressed issues of query-document matching, but the paper does not discuss these prior works in detail. The paper should highlight the unique challenges in DBMS configuration debugging that necessitate novel approaches.}
\end{shaded}

\noindent\textbf{RESPONSE}:
%The unique challenge is that historical questions and DBMS manuals are from different sources, where the semantics may be heterogeneous. 
As suggested, we have revised the Related Work section to include a detailed discussion of traditional IR techniques and highlight the unique challenges. Please see \textbf{M9} for details. 

%To clarify, compared to traditional IR approaches, the unique challenge here lies in retrieving documents from multiple sources, such as historical questions and DBMS manuals, where the semantics of documents from different sources may be heterogeneous. For instance, as illustrated in Figure 2, historical questions typically describe ``what is wrong'' (\eg ``\emph{It takes over 15 minutes\ldots}''), while DBMS manuals focus on ``how to fix it'' (\eg ``\emph{turn off autocommit mode}''). We will expand on this point in the revised Related Work section.
%
%
%Thank you for the suggestion. We will revise the Related Work section to include traditional IR techniques in detail. 
%
%We clarify that, compared with such traditional IR techniques, the unique challenge is that retrieving documents from multiple sources, such as historical questions and DBMS manuals, where the semantics of documents from different sources may be heterogeneous. For example, as shown in Figure 2, historical questions typically describe ``what is wrong'' (e.g., ``It takes over 15 minutes . . .''), while DBMS manuals focus on ``How to fix it'' (e.g., ``turn off autocommit mode'').
%We will discuss this in more detail in the Related Work. 
%
%Please see \textbf{M3 (1)} for details.


\begin{shaded}
\noindent\textit{\textbf{R2O3}: %The effectiveness of the approach heavily relies on the quality and relevance of historical questions, troubleshooting manuals, and telemetry data. 
	(1) Inaccuracies in these sources could lead to incorrect or suboptimal debugging suggestions. 
	(2) Achieving high accuracy in document retrieval among such diverse data types is inherently challenging and can affect overall performance. 
	The paper should discuss (if possible empirically) the sensitivity of the approach to these factors.
}
\end{shaded}

\noindent\textbf{RESPONSE}: Thanks for pinpointing these crucial factors.

(1) We agree that inaccuracies in sources of historical questions, troubleshooting manuals and telemetries can significantly impact overall performance. As suggested, we have added new experiments to empirically investigate these factors. 
%For instance, we plan to introduce noise into the ground-truth labels of historical questions and troubleshooting manuals to evaluate the sensitivity of our approach. 
Please see \textbf{M4} for details. 

(2) We have already explored the impact of document retrieval on overall performance in \textbf{Section~\ref{sec:exp-doc}}. Our results show that the effectiveness of document retrieval significantly affects the overall performance. For example, our proposed retrieval method, which combines different types of documents, not only achieves better retrieval performance (i.e., higher recall) but also enhances overall results compared to using a single type of document.
%, as shown in Figures 7 and 8. 

%We will add a more detailed analysis in this section.

%Thanks for the suggestions. We agree that the effectiveness of the approach heavily relies on the quality and relevance of historical questions, troubleshooting manuals, and telemetry data. To show this point, we will add an experiment to discuss the sensitivity by adjusting the completeness of sources. More details can be referred to \textbf{M2 (5)}. 

\begin{shaded}
\noindent\textit{\textbf{R2O4}: %Analyzing telemetry data involves understanding a wide array of metrics, which can be complex and slow. 
	(1) The paper should provide more details on the scalability of the approach (both in number and types) for detecting relevant telemetries. (2) it should address whether telemetries are "always" necessary, what queries benefit more telemetries, and what happens when there is ambiguity.}
\end{shaded}

\noindent\textbf{RESPONSE}: (1) As suggested, we have added a new experiment to examine the scalability of our approach for detecting relevant telemetry data in \textbf{Section~\ref{sec:exp-eff}}. Specifically, we have varied the number of input metrics and differentiate between metric types, and report the time required for telemetry data analysis. 
Please refer to \textbf{M5}. 

(2) We have already analyzed the impact of telemetry data in \textbf{Section~\ref{sec:exp-tel}}. Our experimental results suggest that telemetry data may not ``always'' be necessary, as shown in \textbf{Figure~\ref{fig:type}}. Specifically, compared to \sys-docs-only (i.e., without telemetry data), \sys does not always demonstrate superior performance. This is because some anomalies are not caused by anomalous resource usage, such as the error ``\emph{column `DateReceived' cannot be null}'' shown in \textbf{Figure~\ref{fig:overview}}. Additionally, we found that queries involving tuning numerical knobs tend to benefit more from telemetry data. We have revised \textbf{Section~\ref{sec:exp-tel}} to provide a more detailed analysis.


%We will add a telemetry scale sensitivity experiment to analyze the impact of telemetry data size on running time. Please see \textbf{M2 (6)} for details. Actually, the telemetries may not ``always'' be necessary because some anomalies are not caused by the anomalous resources usage, such as the error ``The column `DateRecieved' cannot be null'' in Figure 1, and we have discussed it in Exp-4 in detail.

\begin{shaded}
\noindent\textit{\textbf{R2O5}: %Overall, the results appear to be on the lower end (with F1 score over < 0.50). 
	The paper should explain why these results are statistically significant (e.g, how does it significantly reduces the operational burden) compared to the option of having a DBA search discussion or community forums. 
	Furthermore, %it might help to 
 discuss how the provided results by \sys can be trusted w/o significant troubleshooting.}
\end{shaded}

\noindent\textbf{RESPONSE}:
We have conducted a new experiment to evaluate whether \sys offers a statistically significant advantage over DBAs searching through discussion or community forums in \textbf{Section~\ref{sec:exp-eff}}.
%
%evaluate the time taken by DBAs to solve problems with and without \sys, in order to determine whether \sys offers a statistically significant advantage over DBAs searching through discussion or community forums. 
Please see \textbf{M3} for details.

We have also added a discussion in \textbf{Section~\ref{sec:framework}} on how \sys can be trusted. The key idea is that \sys not only provides configuration recommendations but also offers \emph{explanations}, grounded in historical questions, troubleshooting manuals, and telemetry data. 
%We will also revise Figure 2 to illustrate the explanations. 

%In the NL setting, it requires that the output knobs must be strictly the same as the answer, while ignoring some other knobs that may be valid. This is the reason for the low F1-score and why we propose the Runnable setting. To explain why these results are statistically significant, we add an experiment to quantify the time cost of DBA to solve problems (see \textbf{M2 (3)}). Moreover, we will add case studies to our experiments to show how \sys works and the improvement room. Please see M1 for details.

%
%\stitle{Required Changes: }
%
%\begin{shaded}
%\noindent\textit{\textbf{R2C1}: Dig more into the details on %experiments \ldots% to help understand the result. Please 01.
%}
%\end{shaded}
%
%\noindent\textbf{RESPONSE}: %We will add more experiments %and discussion about our results (
%Please see our responses to \textbf{R2O1}.
%
%\begin{shaded}
%\noindent\textit{\textbf{R2C2}: Provide more details on how %the approach scales in capturing telemetry %data/characteristics. %Please 04.
%}
%\end{shaded}
%
%\noindent\textbf{RESPONSE}: %We will add a telemetry scale sensitivity experiment to analyze the impact of telemetry data size on running time. 
%Please see our responses to \textbf{R2O4}.

%\begin{shaded}
%\noindent\textit{\textbf{R2C3}: Briefly compare and constrast with existing body of research query-document matching, highlighting characteristics of problem that necessisates a new approach the paper proposes. %Please see O2.
%}
%\end{shaded}

%\noindent\textbf{RESPONSE}: %We will discuss it more clearly in the related work of our paper. 
%Please see our responses to \textbf{R2O2}. 

%\begin{shaded}
%\noindent\textit{\textbf{R2C4}: Not a must but also see if O3 and P5.}
%\end{shaded}
%
%\noindent\textbf{RESPONSE}: %We will address these concerns as 
%Please see our responses to \textbf{R2O3} and \textbf{R2O5}. 

\vspace{-1em}
\section*{Responses to Reviewer \#3}

\begin{shaded}
\noindent\textit{\textbf{R3O1}: %While it make sense that LLMs can help identify relevant configuration knobs, 
the intuition why it is a good candidate for recommending knob values is not as clear. LLMs are not particularly good at numerics. I wonder why the problem setup chooses to directly output the knob value, instead of suggesting directional adjustments (e.g., increase/decrease, enable/disable).}
\end{shaded}

\noindent\textbf{RESPONSE}: 
We have included a detailed discussion in \textbf{Section~\ref{sec:framework}} to justify the intuition why LLM is good for recommending knob values. Please see \textbf{M10} for details. 
%
The reason why we directly output the knob value is that it is more convenient for the user to set an exact value than suggesting directional adjustments. For example, if \sys recommends the user to increase a knob, user may still not know which value is suitable. 

%We agree that LLMs are not particularly good at numerics because the value setting depends on the runnable environment and cannot be solved simply by LLM using documentation or experience. As a result, there exists more optimization. We will explain it clearer in our future work. 

%

\begin{shaded}
\noindent\textit{\textbf{R3O2}: %In addition to telemetry data, 
it seems like statistics on the sql table, statistics of query workload and machine resources such as memory size could also play a role in debugging. 
%For example, physical memory of the machine could affect knob choices such as buffer pool or table size.
}
\end{shaded}

\noindent\textbf{RESPONSE}: 
%We agree that these statistics play a role in debugging. 
% We have conducted new experiments to evaluate the impact of these statistics. 
% Please see \textbf{M7} for details.
We have conducted new experiments to investigate the impact of providing additional contextual information to prompt the LLM, specifically focusing on \emph{DB statistics from the tables}. We utilize the table names, the number of tuples, column names, and column data types as the DB statistics. We added this information to origin \sys and use GPT 3.5 to evaluate it. The accuracy of dataset ``MySQL Run'' in Runnalbe setting is $0.61$, which is lower than \sys (0.79). 
These results suggest that the current three sources, \ie historical questions, DBMS manuals, and telemetry, seem sufficient, and adding more information for the LLM may adversely affect its predictions.


%We infer that the current three sources (historical questions, DBMS manuals and telemetry) are sufficient, and providing more information for the LLM may actually affect its predictions.

%
%As some statistics (query workload and machine resources are included in telemetry), we will add DB statistics from the tables as a new source for \sys in the experiment to verify this claim. Please see \textbf{M2 (2)} for details.

\begin{shaded}
\noindent\textit{\textbf{R3O3}: %With only a few hundred training data points, it’s unsurprising that the PLM baseline shows very poor performance. 
This PLM baseline could be made stronger if you augment the training data using examples generated from Section~\ref{sec:da}.}
\end{shaded}

\noindent\textbf{RESPONSE}: We have added this baseline in the revised version, as described in \textbf{M1}.

%augment the training data for PLM as a new baseline. Please see \textbf{M2 (1)} for more details.

\begin{shaded}
\noindent\textit{\textbf{R3O4}: It would also help to get some idea on the coverage of the evaluation datasets. What percent of MySQL/Postgres knobs were covered in the documentation, manual and test datasets?}
\end{shaded}

\noindent\textbf{RESPONSE}: 
%Thanks for the suggestions. 
We have discussed the coverage of the evaluation datasets in \textbf{Section~\ref{sec:exp-setup}}, as described in \textbf{M7}.

%add these statistics (knob coverage in training questions, historical questions, manuals and test questions) in our experiments. Please see \textbf{M2 (7)}.

\stitle{Minor remarks}:

\begin{shaded}
\noindent\textit{\textbf{R3C1}: Numeric knobs have higher success rate than categorical ones (Figure 9). Does it mean that the specific values of numeric knobs do not matter that much - multiple values would work.}
\end{shaded}

\noindent\textbf{RESPONSE}: Yes, multiple values would work. %In many cases, correctly choosing to lower/raise the knob value may solve the user's questions. 
We have explained this in the case study (see \textbf{M12}).

% \vspace{-1em}
\begin{shaded}
\noindent\textit{\textbf{R3C2}: It wasn't clear until the evaluation that there are essentially two version of \sys. One is only concerned with identifying the correct subset of the knobs and does not predict knob values (the NL setting). The other takes telemetry data and also predicts knob values (the Runnable setting).}
\end{shaded}

\noindent\textbf{RESPONSE}: Thanks. We have clarified it when introducing the framework in \textbf{Section~\ref{sec:framework}}.

\begin{shaded}
\noindent\textit{\textbf{R3C3}: In section~\ref{sec:exp-tel} “ (2) \sys-telemetry-only: \sys without telemetry data analysis, (3) \sys- docs-only: \sys without document retrieval”. Is this a typo? 
%Does “\sys-telemetry-only” mean \sys with telemetry data analysis?
}
\end{shaded}

\noindent\textbf{RESPONSE}: We have fixed it. Thanks!

%
%\begin{shaded}
%\noindent\textit{\textbf{Required Changes}: O1-O4}
%\end{shaded}
%
%\noindent\textbf{RESPONSE}: We will address all concerns in %O1-O4.
%

% \vspace{-1em}
\section*{Responses to Meta Reviewer}
 
\begin{shaded}
\noindent\textit{\textbf{C1}: (1)The reviewers felt the experiments warranted more specific motivations — characterizing the types of queries for which these techniques are (and are not) effective, and assessing the sensitivity of these methods to question frequency in the training data. (2) Providing experiments to show more specifically where the proposed approach does or does not excel would provide a more nuanced recommendation for practitioners — some results are modest, and limitations are not discussed.}
\end{shaded}

\noindent\textbf{RESPONSE}:
(1) Please refer to our responses to \textbf{R2O1}. (2) See our responses to \textbf{R1O4} and \textbf{R2O5}.
% As discussed in \textbf{R2O1}, we have conducted a sensitivity analysis in Figure 7, Figure 8 and Figure 9. And we will add more case studies (see \textbf{M1}) in our experiments to show why \sys works and what is the room to improve.

\begin{shaded}
\noindent\textit{\textbf{C2}: (1) The reviewers also noted that the experiments are limited to a small dataset, which puts competitive methods at a disadvantage. If this limited dataset is realistic, some additional motivation is warranted. Otherwise, increasing its size to provide a more realistic setting for competitive methods would make the argument more convincing. (2) A related issue is the availability of training labels — the cost in time and training warrants additional discussion. (3) In addition, providing more baselines involving LLMs (e.g., varying prompting, fine-tuning, or other setups). Your shepherd can assist with considering additional experiments and discussion.}
\end{shaded}

\noindent\textbf{RESPONSE}: 
(1) We have increased the dataset size. Please refer to \textbf{M2}. (2) Please refer to our responses to \textbf{R1O2}. (3) We will add these baselines in the experiments. Please refer to \textbf{M1}.
%We will increase the size of the dataset in the Runnable setting. Please see details in \textbf{M2 (8)}. For the availability of training labels, the labeling process is automated and does not cost much time. Please see \textbf{M3 (3)} for details. We will clarify this in our paper. In addition, we will add more baselines as we discussed in \textbf{M2 (1)}.

\begin{shaded}
\noindent\textit{\textbf{C3}: (1) There was also consensus that the paper could be significantly improved by highlighting the unique challenges in this context of configuration debugging relative to more general query-document matching in the IR literature, and (2) the generalizability of the system to other DBMS. (3) Also, some design decisions warrant more discussion: The output is numeric settings, but LLMs can struggle with reasoning about numeric values. Therefore some discussion about alternatives, including qualitative adjustments (direction, categorical magnitudes) could produce different results.}
\end{shaded}

\noindent\textbf{RESPONSE}: 
(1) Please refer to our responses to \textbf{R2O2}. (2) Please refer to our responses to \textbf{R1O7} or \textbf{M11}. (3) Please refer to our responses to \textbf{R3O1} or \textbf{M10}.

% As we discussed in \textbf{M3 (1)} and \textbf{R2O2}, the unique challenge is that historical questions and DBMS manuals are from different sources, where the semantics may be heterogeneous. We will discuss it more clearly in related work. For design decisions, as we discussed in \textbf{M3 (2)} and \textbf{R3O1}, compared with qualitative adjustments, directly setting knob value can be more convenient for users and LLM can accomplish value setting by leveraging in-context knowledge and trained knowledge to decide the value. Moreover, we agree that these methods have room for improvement for numeric values, which we will clarify in our future work.

\begin{shaded}
\noindent\textit{\textbf{C4}: %The reviewers felt 
\ldots the results could be improved by providing additional contextual information to the LLM: machine resources, DB statistics from the tables, statistics of the query workload when available. %Some discussion or additional experiments of these effects would help show new directions.
}
\end{shaded}

\noindent\textbf{RESPONSE}:
Please refer to our responses to \textbf{R3O2}
% As discussed in \textbf{M2 (2)} and \textbf{R3O2}, we will add DB statistics from the tables as a new source for \sys in the experiment and discuss the results.  


\begin{shaded}
\noindent\textit{\textbf{Required Changes}: Overall: R1O1, R1O2, R1O4, R1O7, R2O1, R2O2, R2O4, R3O1, R3O3; Optional changes include R103, R1O5, R1O6, R1O8, R2O3, R3O2}
\end{shaded}

\noindent\textbf{RESPONSE}: We have addressed all the concerns.




==> response/revision-plan-bak.tex <==


\subsection*{Dear SIGMOD Meta-Reviewer and Reviewers,}

\noindent 
Thank you for your thoughtful reviews and encouraging comments. We will use your feedback to make significant revisions to our paper. Below, we have summarized our revision plan and provided responses to each reviewer.

\section*{Revision Plan}
\stitle{M1 [New Case Studies]}: We will conduct case studies where we sample user questions that Andromeda successfully addressed, as well as cases where Andromeda failed, and analyze how Andromeda works and the room for improvement.
%We have conducted sensitivity experiments of different queries' knob type and queries' knob frequency in Figure 7, Figure 8 and Figure 9. If more sensitivity experiments are needed, we can add them when revising the paper. Moreover, we will conduct case studies to show which queries are successfully solved and which are failed with analyzing the reasons.
 
\stitle{M2 [New Experiments]}: We will conduct new experiments:
\begin{enumerate}
    \item
    \textbf{More baselines}: For PLM, we will use the same training method of PLM with augmented training data (\textbf{DA + PLM}). For LLM, we will add the following baselines.
 \textbf{(a) More models:} add more large language models to replace GPT in our existing experiments. Specifically, we use Qwen, Llama-3 to replace GPT with the following baselines - \textbf{Qwen, Llama-3, Qwen (all knobs), Llama-3 (all knobs)}. Moreover, we also replace GPT in Andromeda as Andromeda-Qwen, Andromeda-Llama-3. 
\textbf{(b) Varying prompts}: add more prompt engineering techniques(CoT, task decompose). 
\textbf{(c) Fine-tuning}: fine-tune GPT 3.5 using the training data.
 \item \textbf{More retrieval sources}: We will evaluate the overall quality after adding DB statistics from the tables. In particular, we use a template to transfer DB statistics into a text description. Then we add it to Andromeda's prompt (containing historical questions, manuals and telemetries) and evaluate the reasoning results, comparing it with original Andromeda.
 \item \textbf{Time cost quantification}: We will add a user study to evaluate Andromeda's time cost. Specifically, we will first invite two experienced DBAs to manually solve the problems with provided historical questions, database manuals and telemetries and record the time cost. Second, we will ask two other experts with the equivalent ability to solve the problem using Andromeda and record the time cost. Finally, we will compare these two records to show how Andromeda works.

 \item \textbf{Adding recall / precision results}: We will add recall /precision scores in the NL setting for the overall evaluation.
\item \textbf{Sensitivity of source quality}: We use the completeness of the included knobs to indicate the quality of the source. We will add a sensitivity experiment to reduce the knobs contained in the source to evaluate the impact of different source quality on Andromeda performance.

\item \textbf{Sensitivity of telemetry scale}: We will analyze different scales of telemetry by gradually reducing the metric types and timestamps and evaluate their results.

\item \textbf{Adding statistics}: we will add more statistics, including knob coverage in training questions, historical questions, manuals, and test questions.
% We will add more statistics including knob coverage in training questions, historical questions, manuals, and test questions.

\item \textbf{Dataset}: For the NL setting, we have obtained almost all knob configuration-related questions in StackOverflow dataset and MySQL community, it is hard to scale. For the runnable setting, we will add more questions to around 100.

\end{enumerate}

\stitle{M3 [Clarifications]}: We will make the following clarifications:

\begin{enumerate}
    \item \textbf{Compared with IR literature}: Generally speaking, existing IR algorithms aim to match queries and documents. There are three challenges in the DBMS configuration scenario. 
    (i) The semantics of documents from different sources may be heterogeneous. For example, historical questions typically describe ``what is wrong'', while DBMS manuals focus on ``How to fix it''. 
    (ii) For existing IR algorithms, there is a lack of sufficient high-quality training data for DBMS configuration problem. 
    (iii) It is hard for existing IR algorithms to analyze telemetry data. In general, DBMS configuration requires reasoning and cannot be solved by direct text matching.

    \item \textbf{Reasoning configuration value}: There are two reasons why LLMs work. 
    (i) Using RAG, LLM can obtain knowledge about the knobs. For example, LLM can set autocommit=0 with manual "when importing data into InnoDB, turn off autocommit mode, because…", and it can set $innodb\_log\_file\_size=256M$ if the similar question sets the same value. 
    (ii) LLMs may learn some common settings in pre-training or finetuning phase. Moreover, we agree that we need more techniques to optimize the configuration value reasoning using LLM such as dealing numeric value more smartly. We will explain it in our future work. 

    \item \textbf{Automating training label}:  The training label can be automated annotated. For the real training data, we use regular expressions to match related knobs from accepted answers or comments of questions. For augmented training data, we generate questions based on a knob’s manual, and this knob is the label corresponding to the questions. We will explain it more clearly in our paper.
\end{enumerate}



\section*{Responses to Reviewer \#1}

\begin{shaded}
\noindent\textit{\textbf{R1O1}: Experimental eval should include a few other baselines that use LLMs for solving the same problem\ldots}
\end{shaded}

\noindent\textbf{RESPONSE}: Thanks for the suggestion. To the best of our knowledge, we are the first to develop an LLM-based DBMS diagnosis system designed to accept NL questions on DBMS configuration issues and recommend specific configurations to address the issues. Therefore, to address the concern, we can only add more baselines by replacing GPT with other LLMs, \eg Qwen and Llama-3. Please see \textbf{M2 (1)} in our revision plan for more details.

\begin{shaded}
\noindent\textit{\textbf{R1O2}: There seems to be a lot of human effort required in collecting ground labels for training and evaluation (including confirmation by experts). Human in the loop in ML requires non-trivial amount of time and dollar cost. More discussion is needed.}
\end{shaded}

\noindent\textbf{RESPONSE}: Sorry for the confusion. We clarify that Andromeda does not require significant human effort to collect ground labels for training and evaluation due to its automated labeling process. Please see \textbf{M3 (3)} for details. Moreover, to validate the labeling quality, we have randomly sampled some training and testing cases for manual verification, which have confirmed that our automatic labeling method is reasonable.

\begin{shaded}
\noindent\textit{\textbf{R1O3}: Related to the above point, the goal of Andromeda is to reduce the time it takes to manually arrive at a solution by expert DBAs. How could the paper quantify this claim?}
\end{shaded}

\noindent\textbf{RESPONSE}: We will add a user study to evaluate the time cost of DBAs to solve problems with / without Andromeda, so as to quality how \sys reduces the time. Please see \textbf{M2 (3)} for details.
 
\begin{shaded}
\noindent\textit{\textbf{R1O4}: the overall F-1 scores from Table 2 are still not very high for Andromeda. There seems to be a lot of room for improvement.}
\end{shaded}

\noindent\textbf{RESPONSE}: We first explain why the overall F-1 scores from Table 2 are not very high for \sys. As introduced in Section 6.1, the evaluation in the NL setting requires that \sys's output knobs strictly match the automatically labeled answers, while disregarding other potentially valid knobs. This can lead to an underestimation of the F1-score, which is why we proposed the Runnable setting. In the Runnable setting, DBMS experts assess whether the recommended configurations resolve the issues. As shown in Table 2, \sys achieves a SuccessRate of over 0.7.

Moreover, we agree that ``there seems to be a lot of room for improvement'' -- we really hope for a call-to-arms to significantly push this core database problem. To support this effort, we will conduct an in-depth analysis of the bad cases produced by \sys. Please refer to \textbf{M1} for more details.

%In the NL setting, it requires that the output knobs must be strictly the same as the answer, while ignoring some other knobs that may be valid. This is the reason for the low F1-score and why we propose the Runnable setting. To show this, we will add case studies for bad cases. Please see \textbf{M1} for details. We agree that ``there seems to be a lot of room for improvement'' -- we really hope for a call-to-arms 
%to significantly push this core database problem.

\begin{shaded}
\noindent\textit{\textbf{R1O5}: What was the actual prompt submitted to the LLM? It wasn't presented in the main body of the paper.}
\end{shaded}

\noindent\textbf{RESPONSE}: 
Please refer to Figure 2(b) as an illustrative prompt submitted to the LLM. To make it clearer, we will add more real prompts in experiments in case studies (see \textbf{M1}). Moreover, we have already included all the prompts in our experiments in the repo: \url{https://anonymous.4open.science/r/Andromeda-D150/}

\begin{shaded}
\noindent\textit{\textbf{R1O6}: it would also be particularly insightful to discuss some loss cases for Andromeda for which it does not do well and how Andromeda could be improved to address those losses?}
\end{shaded}

\noindent\textbf{RESPONSE}: Thank you for the suggestion. We will include a detailed analysis of the bad cases to highlight the limitations of \sys and discuss potential improvements. Please refer to \textbf{M1} for more details.

\begin{shaded}
\noindent\textit{\textbf{R1O7}: How generalizable is Andromeda to other DBMSes? Would it require training data generation, model training, and evaluation for each DBMS?}
\end{shaded}

\noindent\textbf{RESPONSE}: \sys can be easily generalized to other DBMSes, as the algorithms for training data generation, model training, and evaluation are adaptable to new DBMSes. Specifically, when applying \sys to a new DBMS, all that is required is the specification of the knobs and the manuals of the DBMS. \sys can then use these inputs to automatically generate augmented data and train a new model during the offline stage, while supporting evaluation on the DBMS in the online stage.

% it needs to regenerate augmented data and retrain a new model in the offline stage because different DBMSs contain different knobs and manuals. Nevertheless, the algorithms for DA and training can be generalized.

\begin{shaded}
\noindent\textit{\textbf{R1O8}: The paper talks about the time efficiency of Andromeda but a discussion on the cost efficiency is missing.}
\end{shaded}

\noindent\textbf{RESPONSE}: As suggested, we report the cost efficiency, which is the average cost of calling LLMs for each NL debugging question $q$:  
$0.0017$\$ for GPT-3.5, $0.053$\$ for GPT-4, $0.012$\$ for GPT-3.5 (all knobs), $0.039$\$ for GPT-4 (all knobs), $0.006$\$ for \sys-3.5 and $0.022$\$ for \sys-4. We can see that \sys have good performance on cost efficiency. We will add a report on cost efficiency in the revised version. 
Please see \textbf{Mx} for more details. 

%Thanks for the suggestion. To calculate the cost of each query, we have calculated the average cost of prompt and response respectively and we add the prompt cost and response cost as the cost efficiency. In detail, 
%\begin{itemize}
%    \item GPT-3.5 costs $0.0017$\$ / query. 
%    \item GPT-4 costs $0.053$\$ / query. 
%    \item GPT-3.5 (all knobs) costs $0.012$\$ / query. 
%    \item GPT-4 (all knobs) costs $0.039$\$ / query.
%    \item Andromeda-3.5 costs $0.006$\$ / query.
%    \item Andromeda 4 costs $0.022$\$ / query.
%\end{itemize}

%We will add a more detailed report on the cost efficiency in experiments.

\subsection*{Minor Remarks:}

\begin{shaded}
\noindent\textit{\textbf{R1C1}: It appears all telemetry data is always analyzed in real-time? There seems to be a lot of room for optimization here. %Please comment.
}
\end{shaded}

\noindent\textbf{RESPONSE}: 
Yes, the telemetry data is analyzed in real-time. We have conducted a latency analysis, as reported in Table 8. The result shows that the time used for telemetry analysis is 2.85 seconds, which we believe is acceptable for users. However, we agree that there is room for optimization, such as filtering out unnecessary telemetry data. We will address this in future work.

%Yes, the telemetry data is analyzed in real-time. Actually, we have conducted the latency analysis in Table 8. The time consumption is in seconds, which we think is acceptable to users. In addition, we agree that there exists room for optimization, such as filtering useless telemetry. We will add it in our future work.

\begin{shaded}
\noindent\textit{\textbf{R1C2}: How does Andromeda (and related approaches) deal with cases where a small variation of a question compared to a historical question leads to a very different solution?}
\end{shaded}

\noindent\textbf{RESPONSE}: 
\sys deals with these cases by matching domain-specific contexts from other sources, including troubleshooting manuals and DBMS telemetry data. This is one of the key reasons we use multiple sources in our RAG approach. Specifically, when relying solely on historical questions is not sufficient, prioritizing relevant manuals or telemetry data over potentially confusing historical questions can provide more accurate solutions.


%\sys addresses these cases by matching domain-specific contexts for the question from other sources, including troubleshooting manuals and DBMS telemetries. Actually, this is the key reason that motivates us to use multiple sources for RAG. Specifically, when using single historical questions as sources is not helpful, ranking the helpful manuals/telemetries before this confusing historical question may help.

%For those cases where a small variation of a question compared to a historical question leads to a very different solution, using single historical questions as sources is not helpful. To deal with it, Andromeda uses multiple sources for RAG, for example, ranking the helpful manuals before this confusing historical question can help.

\begin{shaded}
\noindent\textit{\textbf{R1C3}: there could be multiple ways to fix the same issue? It's unclear how Andromeda and related approaches are reasoning about and ranking between different tuning knobs?}
\end{shaded}

\noindent\textbf{RESPONSE}: Yes, there could be multiple ways, such as different tuning knobs, to fix the same issue, as illustrated in Figure 2(b). \sys uses an LLM to reason about the various tuning knobs and select the most appropriate set. Specifically, as discussed in \emph{Step 3} of the online stage in Section 3, \sys generates a prompt that includes all the retrieved data and then calls the LLM to recommend the configurations, i.e., the tuning knobs, to address the issue. We will revise Section 3 to clarify this further.

%
%Yes, there could exist multiple ways, \ie tuning knobs, to fix the same issue, as shown in Figure 2(b). \sys relies on an LLM to reason about between different tuning knobs and identify an appropriate set of knobs. Specifically, as discussed in \emph{Step 3} in the online stage of Section 3, \sys generates an prompt by including all the retrieved data and calls an LLM to generate the configuration recommendations, \ie tuning knobs, to fix the issue. We will revise Section 3 to make it clearer. 

%
%For the reasoning of Andromeda, it outputs the most related knobs using LLM to select knobs from candidate knobs in multi-sources as the top-1 result for the query. 

\begin{shaded}
\noindent\textit{\textbf{R1C4}: %In Sec 4.3, it's unclear by 
	why manual-manual samples are prioritized over others?}
\end{shaded}

\noindent\textbf{RESPONSE}: 
We conducted an experiment to evaluate different prioritization strategies, and the results show that prioritizing manual-manual training samples yields the best performance. The primary reason is that aligning manual-manual samples is ``easier'' than aligning question-question or manual-question samples due to the formality and consistency of manuals. By training our Alignment component on these easier cases first, we ensure it is adequate before gradually improving it on more challenging cases.
%
%We conducted an empirical evaluation of various configurations and found that prioritizing manual-manual samples yields the best quality. Our analysis suggests that optimizing models individually first benefits joint training. Specifically, optimizing the manual embedding model with manual-manual samples and the question embedding model with question-question samples leads to better performance when training multiple models using question-manual samples.
% Manual-manual samples are prioritized over others, because training manual-manual samples is the basis for training question-manual / manual-question samples. Given a question, the target of training manual-manual samples is to correctly represent manuals in hidden space to deal with multi-source heterogeneity. And after manuals currently embedded, Andromeda should learn to adjust question and manual embeddings based on the trained manual embeddings. 


\begin{shaded}
\noindent\textit{\textbf{R1C5}: %The document embeddings are stored in a vector DB. May be some quick mention of 
	what kind of vector DB and what kind of and size of indexes are needed to meet the runtime SLA of Andromeda?}
\end{shaded}

\noindent\textbf{RESPONSE}: We use Meta Faiss as our vector database to index the embeddings of historical questions and manuals. In the current implementation of \sys, we have indexed 5,138 vectors for MySQL and 1,158 vectors for PostgreSQL, with each vector having a dimension of 768. We will clarify this further in the paper.

\begin{shaded}
\noindent\textit{\textbf{R1C6}: Analyzing a large amount of telemetry data and zooming in on the sections that might be correlated with the issue being debugged does not seem to be a new challenge and there may already be existing approaches.}
\end{shaded}

\noindent\textbf{RESPONSE}: 
There are two key challenges that distinguish our work. First, detecting anomalous telemetry data from vast amounts of time-series information is particularly difficult due to the influence of seasonality and trends, which can obscure what is truly anomalous. Second, existing approaches do not address the semantic correlation between natural language queries and telemetry data, an essential aspect of our solution.
% There are two new challenges: The first challenge is detecting anomalous telemetries from a huge amount of time-series data, as it is not easy to identify what is anomalous with the influence of sessonal and trand. Secondly, existing works do not consider the sematic correlation of the NL query and telemetries.
% We are the first to deal with user database diagnosis text questions using telemetry data. In detail, existing works analyze telemetry through only one aspect (such as the d-bot use rule to detect anomaly in telemetry). In contrast, our work comprehensively analyzes telemetry from multiple aspects that are anomalies in time series data of metric, the correlation of query and metrics with the description of metrics in manual. 

\begin{shaded}
\noindent\textit{\textbf{Required Changes}: O1, O2, O4, O6, O8 (and addressing minor comments)}
\end{shaded}

\noindent\textbf{RESPONSE}: We have addressed all concerns. Please see our responses mentioned above.

\section*{Responses to Reviewer \#2}

\begin{shaded}
\noindent\textit{\textbf{R2O1}: The experimental setup and findings lack sufficient details \ldots
	 %to aid understanding. For example, 
	 (1) the paper should explore which types of queries LLMs perform well on, where RAG helps, and whether historical queries can be categorized by type and frequency. It should also examine how the system performs for queries with less frequent questions. 
	 %
	 (2)Including results on precision and recall in Table 2 would also help.}
\end{shaded}

\noindent\textbf{RESPONSE}: 
Thank you for the suggestion. We will revise the paper by provide more details of experimental setup and findings.

(1) We have already categorized queries by considering the frequency and types of their ground-truth labels (i.e., the tuning knobs). Specifically, as shown in Figures 7 and 8, we classify queries into high-, medium-, and low-frequency categories. We have also explored the questions raised by the reviewer. For instance, in most cases, LLMs perform better on high-frequency queries compared with medium- and low-frequency ones, while RAG consistently improves performance across all frequency levels. Additionally, we have examined \sys's performance on less frequent queries. In Figure 9, we further categorize queries by the type of their corresponding knobs (i.e., numerical, categorical, and boolean). Our findings show that \sys achieves better performance on numerical and boolean queries compared to categorical ones. We will revise the paper to include detailed explanations of these experimental setups and findings.

(2) As suggested, we will include precision and recall results in Table 2 to make the comparison more comprehensive.


%Thanks for the suggestions. As discussed in \textbf{M1}, We have conducted sensitivity experiments of the type of knob in different queries and the frequency of the knob in the queries in Figure 7, Figure 8 and Figure 9. If more sensitivity experiments are needed, we can add them when revising the paper. Moreover, we will conduct case studies (see \textbf{M1})to show which queries are successfully solved and which are failed in analyzing the reasons. And we will add recall / precision in Table 2.

\begin{shaded}
\noindent\textit{\textbf{R2O2}: Traditional IR techniques have long addressed issues of query-document matching, but the paper does not discuss these prior works in detail. The paper should highlight the unique challenges in DBMS configuration debugging that necessitate novel approaches and solutions.}
\end{shaded}

\noindent\textbf{RESPONSE}:
%The unique challenge is that historical questions and DBMS manuals are from different sources, where the semantics may be heterogeneous. 
The unique challenge is that retrieving documents from multiple sources, such as historical questions and DBMS manuals, where the semantics of documents from different sources may be heterogeneous. For example, as shown in Figure 2, historical questions typically describe ``what is wrong'' (e.g., ``It takes over 15 minutes . . .''), while DBMS manuals focus on ``How to fix it'' (e.g., ``turn off autocommit mode'').
We will discuss this in more detail in related work. And please see \textbf{M3 (1)} for details.


\begin{shaded}
\noindent\textit{\textbf{R2O3}: The effectiveness of the approach heavily relies on the quality and relevance of historical questions, troubleshooting manuals, and telemetry data. Inaccuracies in these sources could lead to incorrect or suboptimal debugging suggestions. Achieving high accuracy in document retrieval among such diverse data types is inherently challenging and can affect overall performance. The paper should discuss (if possible empirically) the sensitivity of the approach to these factors.}
\end{shaded}

\noindent\textbf{RESPONSE}: Thanks for the suggestions. We agree that the effectiveness of the approach heavily relies on the quality and relevance of historical questions, troubleshooting manuals, and telemetry data. To show this point, we will add an experiment to discuss the sensitivity by adjusting the completeness of sources. More details can be referred to \textbf{M2 (5)}. 

\begin{shaded}
\noindent\textit{\textbf{R2O4}: Analyzing telemetry data involves understanding a wide array of metrics, which can be complex and slow. The paper should provide more details on the scalability of the approach (both in number and types) for detecting relevant telemetries. Additionally, it should address whether telemetries are "always" necessary, what queries benefit more telemetries, and what happens when there is ambiguity.}
\end{shaded}

\noindent\textbf{RESPONSE}: Thanks for the suggestions. We will add a telemetry scale sensitivity experiment to analyze the impact of telemetry data size on running time. Please see \textbf{M2 (6)} for details. Actually, the telemetries may not ``always'' be necessary because some anomalies are not caused by the anomalous resources usage, such as the error ``The column `DateRecieved' cannot be null'' in Figure 1, and we have discussed it in Exp-4 in detail.

\begin{shaded}
\noindent\textit{\textbf{R2O5}: Overall, the results appear to be on the lower end (with F1 score over < 0.50). The paper should explain why these results are statistically significant (e.g, how does it significantly reduces the operational burden) compared to the option of having a DBA search discussion or community forums. Furthermore, it might help to discuss how the provided results by Andromeda can be trusted w/o significant troubleshooting.}
\end{shaded}

\noindent\textbf{RESPONSE}: In the NL setting, it requires that the output knobs must be strictly the same as the answer, while ignoring some other knobs that may be valid. This is the reason for the low F1-score and why we propose the Runnable setting. To explain why these results are statistically significant, we add an experiment to quantify the time cost of DBA to solve problems (see \textbf{M2 (3)}). Moreover, we will add case studies to our experiments to show how Andromeda works and the improvement room. Please see M1 for details.

\subsection*{Required Changes: }

\begin{shaded}
\noindent\textit{\textbf{R2C1}: Dig more into the details on experiments to help understand the result. Please 01.}
\end{shaded}

\noindent\textbf{RESPONSE}: We will add more experiments and discussion about our results (see our response to \textbf{R2O1}).

\begin{shaded}
\noindent\textit{\textbf{R2C2}: Provide more details on how the approach scales in capturing telemetry data/characteristics. Please 04.}
\end{shaded}

\noindent\textbf{RESPONSE}: We will add a telemetry scale sensitivity experiment to analyze the impact of telemetry data size on running time. Please see our response to \textbf{R2O4}.

\begin{shaded}
\noindent\textit{\textbf{R2C3}: Briefly compare and constrast with existing body of research query-document matching, highlighting characteristics of problem that necessisates a new approach the paper proposes. Please see O2.}
\end{shaded}

\noindent\textbf{RESPONSE}: We will discuss it more clearly in the related work of our paper. Please see our response to \textbf{R2O2}. 

\begin{shaded}
\noindent\textit{\textbf{R2C4}: Not a must but also see if O3 and P5.}
\end{shaded}

\noindent\textbf{RESPONSE}: We will address these concerns as our responses to \textbf{R2O3} and \textbf{R2O5}. 


\section*{Responses to Reviewer \#3}

\begin{shaded}
\noindent\textit{\textbf{R3O1}: While it make sense that LLMs can help identify relevant configuration knobs, the intuition why it is a good candidate for recommending knob values is not as clear. LLMs are not particularly good at numerics. I wonder why the problem setup chooses to directly output the knob value, instead of suggesting directional adjustments (e.g., increase/decrease, enable/disable).}
\end{shaded}

\noindent\textbf{RESPONSE}: Using LLMs to predict knob value makes sense because LLM can not only utilize the in-context knowledge with RAG but also some database related knowledge in the pre-training / fine-tuning process, which is helpful for knob value decisions. Please see \textbf{M3 (2)} for details. We agree that LLMs are not particularly good at numerics because the value setting depends on the runnable environment and cannot be solved simply by LLM using documentation or experience. As a result, there exists more optimization. We will explain it clearer in our future work. The reason why we directly output the knob value is that it is more convenient for the user to set an exact value than suggesting directional adjustments. For example, if Andromeda recommends the user to increase a knob, user may still not know which value is suitable.

\begin{shaded}
\noindent\textit{\textbf{R3O2}: In addition to telemetry data, it seems like statistics on the sql table, statistics of query workload and machine resources such as memory size could also play a role in debugging. For example, physical memory of the machine could affect knob choices such as buffer pool or table size.}
\end{shaded}

\noindent\textbf{RESPONSE}: We agree that these statistics play a role in debugging. As some statistics (query workload and machine resources are included in telemetry), we will add DB statistics from the tables as a new source for Andromeda in the experiment to verify this claim. Please see \textbf{M2 (2)} for details.

\begin{shaded}
\noindent\textit{\textbf{R3O3}: With only a few hundred training data points, it’s unsurprising that the PLM baseline shows very poor performance. This baseline could be made stronger if you augment the training data using examples generated from Section 4.2.}
\end{shaded}

\noindent\textbf{RESPONSE}: Thanks for the good suggestions. We will add DA+PLM as a new baseline. Please see \textbf{M2 (1)} for more details.

\begin{shaded}
\noindent\textit{\textbf{R3O4}: It would also help to get some idea on the coverage of the evaluation datasets. What percent of MySQL/Postgres knobs were covered in the documentation, manual and test datasets?}
\end{shaded}

\noindent\textbf{RESPONSE}: Thanks for the suggestions. We will add these statistics (knob coverage in training questions, historical questions, manuals and test questions) in our experiments. Please see \textbf{M2 (7)}.

\stitle{Minor remarks}:

\begin{shaded}
\noindent\textit{\textbf{R3C1}: Numeric knobs have higher success rate than categorical ones (Figure 9). Does it mean that the specific values of numeric knobs do not matter that much - multiple values would work.}
\end{shaded}

\noindent\textbf{RESPONSE}: Yes, multiple values would work. In many cases, correctly choosing to lower/raise the knob value may solve the user's questions. We will explain this in the case study (\textbf{M1}).

\begin{shaded}
\noindent\textit{\textbf{R3C2}: It wasn’t clear until the evaluation that there are essentially two version of ANDROMEDA. One is only concerned with identifying the correct subset of the knobs and does not predict knob values (the NL setting). The other takes telemetry data and also predicts knob values (the Runnable setting).}
\end{shaded}

\noindent\textbf{RESPONSE}: Thanks. We will clarify it when introducing the framework in Section 3.

\begin{shaded}
\noindent\textit{\textbf{R3C3}: In section 6.4 “ (2) Andromeda-telemetry-only: Andromeda without telemetry data analysis, (3) Andromeda- docs-only: Andromeda without document retrieval”. Is this a typo? Does “Andromeda-telemetry-only” mean Andromeda with telemetry data analysis?}
\end{shaded}

\noindent\textbf{RESPONSE}: Will fix. Thanks!

\begin{shaded}
\noindent\textit{\textbf{Required Changes}: O1-O4}
\end{shaded}

\noindent\textbf{RESPONSE}: We will address all concerns in O1-O4.

\section*{Responses to Meta Reviewer}
 
\begin{shaded}
\noindent\textit{\textbf{Required Change C1}: The reviewers felt the experiments warranted more specific motivations — characterizing the types of queries for which these techniques are (and are not) effective, and assessing the sensitivity of these methods to question frequency in the training data. Providing experiments to show more specifically where the proposed approach does or does not excel would provide a more nuanced recommendation for practitioners — some results are modest, and limitations are not discussed.}
\end{shaded}

\noindent\textbf{RESPONSE}: As discussed in \textbf{R2O1}, we have conducted a sensitivity analysis in Figure 7, Figure 8 and Figure 9. And we will add more case studies (see \textbf{M1}) in our experiments to show why Andromeda works and what is the room to improve.

\begin{shaded}
\noindent\textit{\textbf{Required Change C2}: The reviewers also noted that the experiments are limited to a small dataset, which puts competitive methods at a disadvantage. If this limited dataset is realistic, some additional motivation is warranted. Otherwise, increasing its size to provide a more realistic setting for competitive methods would make the argument more convincing. A related issue is the availability of training labels — the cost in time and training warrants additional discussion. In addition, providing more baselines involving LLMs (e.g., varying prompting, fine-tuning, or other setups). Your shepherd can assist with considering additional experiments and discussion.}
\end{shaded}

\noindent\textbf{RESPONSE}: We will increase the size of the dataset in the Runnable setting. Please see details in \textbf{M2 (8)}. For the availability of training labels, the labeling process is automated and does not cost much time. Please see \textbf{M3 (3)} for details. We will clarify this in our paper. In addition, we will add more baselines as we discussed in \textbf{M2 (1)}.

\begin{shaded}
\noindent\textit{\textbf{Required Change C3}: There was also consensus that the paper could be significantly improved by highlighting the unique challenges in this context of configuration debugging relative to more general query-document matching in the IR literature, and the generalizability of the system to other DBMS. Also, some design decisions warrant more discussion: The output is numeric settings, but LLMs can struggle with reasoning about numeric values. Therefore some discussion about alternatives, including qualitative adjustments (direction, categorical magnitudes) could produce different results.}
\end{shaded}

\noindent\textbf{RESPONSE}: As we discussed in \textbf{M3 (1)} and \textbf{R2O2}, the unique challenge is that historical questions and DBMS manuals are from different sources, where the semantics may be heterogeneous. We will discuss it more clearly in related work. For design decisions, as we discussed in \textbf{M3 (2)} and \textbf{R3O1}, compared with qualitative adjustments, directly setting knob value can be more convenient for users and LLM can accomplish value setting by leveraging in-context knowledge and trained knowledge to decide the value. Moreover, we agree that these methods have room for improvement for numeric values, which we will clarify in our future work.

\begin{shaded}
\noindent\textit{\textbf{Required Change C4}: The reviewers felt the results could be improved by providing additional contextual information to the LLM: machine resources, DB statistics from the tables, statistics of the query workload when available. Some discussion or additional experiments of these effects would help show new directions.}
\end{shaded}

\noindent\textbf{RESPONSE}: As discussed in \textbf{M2 (2)} and \textbf{R3O2}, we will add DB statistics from the tables as a new source for Andromeda in the experiment and discuss the results.  


\begin{shaded}
\noindent\textit{\textbf{Required Changes}: Overall: R1O1, R1O2, R1O4, R1O7, R2O1, R2O2, R2O4, R3O1, R3O3; Optional changes include R103, R1O5, R1O6, R1O8, R2O3, R3O2}
\end{shaded}

\noindent\textbf{RESPONSE}: We will address all the concerns (both required and optional) of all reviewers.




==> response/revision-plan.tex <==


\subsection*{Dear SIGMOD Meta-Reviewer and Reviewers,}

\noindent 
Thank you for your thoughtful reviews and encouraging comments. We will use your feedback to make significant revisions to our paper. 
Below, we will first summarize the \textbf{main changes} in our revision plan, followed by \textbf{detailed responses} to each reviewer.

%\section*{Revision Plan}
\stitle{M1 [Case Studies]}: We will add detailed case studies to demonstrate not only the user questions that \sys successfully addressed but also some failure cases where \sys did not perform well, followed by an analysis of the limitations of \sys and how \sys can be further improved.

%
%We will conduct case studies, where we sample some user questions that Andromeda successfully addressed, and some cases that Andromeda failed, analyzing how Andromeda works and the room of improvement.



%We have conducted sensitivity experiments of different queries' knob type and queries' knob frequency in Figure 7, Figure 8 and Figure 9. If more sensitivity experiments are needed, we can add them when revising the paper. Moreover, we will conduct case studies to show which queries are successfully solved and which are failed with analyzing the reasons.


\stitle{M2 [More Baselines]}: We will add more baselines to better evaluate \sys. 
(1) For PLMs, we will also augment the training data for the PLM using our proposed techniques in Section 4.2, and introduce a new baseline \textbf{DA + PLM}.
(2) For LLMs, we will add the following new baselines. First, we will replace GPT with other LLMs, \ie using Qwen and Llama-3 for the new baselines, \textbf{Qwen}, \textbf{Llama-3}, \textbf{Qwen (all knobs)}, \textbf{Llama-3 (all knobs)}, \textbf{\sys-Qwen}, and \textbf{\sys-Llama-3}. Second, we will consider baselines with varying prompting techniques, such as chain-of-thought and task decomposition. Third, we will consider fine-tune GPT-3.5 using our training data.

%
%For PLM, we will use the same training method of PLM with augmented training data (\textbf{DA + PLM}). For LLM, we will add the following baselines.
% \textbf{(1) More models:} add more large language models to replace GPT in our existing experiments. Specifically, we use Qwen, Llama-3 to replace GPT with the following baselines - \textbf{Qwen, Llama-3, Qwen (all knobs), Llama-3 (all knobs)}. Moreover, we also replace GPT in \sys as \sys-Qwen, \sys-llama-3. \textbf{(2) Varying prompts}: add more prompt engineers (CoT, task decompose). \textbf{(3) Fine-tuning}: fine-tune GPT 3.5 using the training data.
 
\stitle{M3 [Larger Datasets]}: We will increase the number of test questions to 100 in the Runnable setting. However, it is challenging to expand the datasets in the NL setting, as we have already gathered nearly all knob-configuration-related questions for MySQL and PostgreSQL from StackOverflow and the MySQL forum. \textbf{We would appreciate guidance from the Shepherd on whether this revision is sufficient.}

%, it is hard to scale. For the runnable setting, we will add more questions to around 100.

\stitle{M4 [New Experiments: End-to-end Time Reduction]}:
We will add a new experiment to evaluate whether \sys effectively reduces the end-to-end time (i.e., the operational burden) for DBAs during database configuration debugging. Specifically, we will employ experienced DBAs and provide them with historical questions, database manuals, and telemetry data. We will then consider two settings: (1) "w/o \sys": where DBAs manually search through historical questions, manuals, and related telemetry data to provide diagnostic suggestions for tuning knobs; and (2) "w \sys": where DBAs follow \sys’s recommendations to address the issues. We will compare the average time taken by the DBAs to troubleshoot configuration issues, thereby demonstrating the effectiveness of \sys.

% 
% We will add a user study to evaluate \sys's time cost. Specifically, we will first invite two experienced DBAs to manually solve the problems with provided historical questions, database manuals and telemetries and record the time cost. Second, we will ask two other experts with the same ability to solve the problem using \sys and record the time cost. Finally, we will compare these two records to show how \sys works.

\stitle{M5 [New Experiments: Sensitivity to Noise Sources]}: 
We will conduct new experiments to examine whether inaccuracies in the retrieval sources (\eg, historical questions, troubleshooting manuals and telemetry data) impact the overall performance of \sys. To this end, we will manually inject noise into these sources, such as replacing the ground-truth labels in historical questions or database manuals with incorrect ones at a certain probability (e.g., 10\%). We will then evaluate \sys's performance on both retrieval effectiveness (e.g., recall) and overall performance.

%\sibei{need updated}. We use the completeness of the included knobs to indicate the quality of the source. We will add a sensitivity experiment to reduce the knobs contained in the source to evaluate the impact of different source quality on \sys performance.

\stitle{M6 [New Experiments: Scalability of Telemetry Data Analysis]}: 
We will add new experiments to examine the scalability of our approach for detecting relevant telemetry data. Specifically, we will vary the number of input metrics and differentiate between metric types, and report the time required for telemetry data analysis. 

%
%We will analyze different scales of telemetry by gradually reducing the metric types and timestamps and evaluate their results.

\stitle{M7 [New Experiments: Effect of Additional Contextual Information]}: 
We will conduct new experiments to investigate the impact of providing additional contextual information to prompt the LLM, specifically focusing on \textbf{DB statistics from the tables}. We will then evaluate whether this information is beneficial and analyze the underlying reasons.

\stitle{M8 [New Experiments: Cost Efficiency]}: 
We will report the cost efficiency, which is the average cost of calling LLMs for each NL debugging question $q$:  
$0.0017$\$ for GPT-3.5, $0.053$\$ for GPT-4, $0.012$\$ for GPT-3.5 (all knobs), $0.039$\$ for GPT-4 (all knobs), $0.006$\$ for \sys-3.5 and $0.022$\$ for \sys-4. We can see that \sys has good performance on cost efficiency. 

%
%We will evaluate the overall quality after adding DB statistics from the tables. In particular, we use a template to transfer DB statistics to a text description. Then we add it to \sys's prompt (containing historical questions, manuals and telemetries) and evaluate the reasoning results, comparing it with original \sys.

\stitle{M9 [More In-Depth Experimental Analysis]}:
(1) We will provide more in-depth analysis by categorizing queries by their types and frequency.
%
(2) We will report precision and recall results in Table 2 to make the comparison more comprehensive.
%
(3) We will further discuss the coverage of the evaluation datasets, with a specific focus on the percentage of MySQL/PostgreSQL knobs covered in the documentation, manuals, and test datasets.


%\textbf{(1) Adding recall / precision results}- We will add recall /precision scores in the NL setting for the overall evaluation. \textbf{(2) Adding statistics information} -  We will add more statistics including knob coverage in training questions, historical questions, manuals, and test questions.

\stitle{M10 [More Clarifications on Experimental Setup]}: 
We will provide more clarifications on experimental setup (Section 6.1). Particularly, we will clarify that the training labels can be automatically annotated. For the original training data, we use regular expressions to extract relevant knobs from accepted answers or comments on questions from StackOverflow or the MySQL Forum. For the augmented training data, we generate questions based on a knob's manual, with the knob serving as the label corresponding to the questions.
To validate the labeling quality, we have randomly sampled some training and testing cases for manual verification, which have confirmed that our automatic labeling method is accurate.


\stitle{M11 [Additional Related Works]}: 
We will revise the Related Work section
to include a detailed discussion of traditional IR techniques.
We will also analyze that, compared to traditional IR approaches, the unique challenge here lies in retrieving documents from multiple sources, such as historical questions and DBMS manuals, where the semantics of documents from different sources may be heterogeneous. For instance, in Figure 2, historical questions typically describe ``what is wrong'' (\eg ``\emph{It takes over 15 minutes\ldots}''), while DBMS manuals focus on ``how to fix it'' (\eg ``\emph{turn off autocommit mode}''). Moreover, it is hard for existing IR techniques to analyze telemetry data in the DBMS debugging scenarios.

%
%Generally speaking, existing IR algorithms aim to match queries and documents. There are three challenges in the DBMS configuration scenario. 
%    (i) The semantics of documents from different sources may be heterogeneous. For example, historical questions typically describe ``what is wrong'', while DBMS manuals focus on ``How to fix it''. 
 %   (ii) For existing IR algorithms, there is a lack of sufficient high-quality training data for DBMS configuration problem. 
 %   (iii) It is hard for existing IR algorithms to analyze telemetry data. In general, DBMS configuration requires reasoning and cannot be solved by direct text matching.


 

\stitle{M12 [Clarifications on Design Choices]}: 
We will revise Section 3 to better clarify our design choices, specifically a particular focus on the following aspects.

(1) There could be multiple ways, such as different tuning knobs, to fix the same issue. \sys uses an LLM to reason about the various tuning knobs and select the most appropriate set. Specifically, \sys generates a prompt that includes all the retrieved data and then calls the LLM to recommend the configurations.

(2) We also justify why using LLMs to predict knob value makes sense. There are two main reasons.
(i) Using RAG, LLM can obtain knowledge about the knobs. For example, LLM can set autocommit=0 with manual "when importing data into InnoDB, turn off autocommit mode, because…", and it can set $innodb\_log\_file\_size=256M$ if the similar question sets the same value. 
(ii) LLMs may learn some database related knowledge in pre-training or fine-tuning process, which is helpful for knob value decisions.
%
Moreover, we agree that we need more techniques to optimize the configuration value reasoning using LLM such as dealing with numeric value more smartly. We will explain it in our future work. 

%
%because LLM can not only utilize the in-context knowledge with RAG but also some database related knowledge in the pre-training / fine-tuning process, which is helpful for knob value decisions.
%Clarification on reasoning configuration value
%There are two reasons why LLMs work. 
%    (i) Using RAG, LLM can obtain knowledge about the knobs. For example, LLM can set autocommit=0 with manual "when importing data into InnoDB, turn off autocommit mode, because…", and it can set $innodb\_log\_file\_size=256M$ if the similar question sets the same value. 
%    (ii) LLMs may learn some common settings in pre-training or finetuning phase. Moreover, we agree that we need more techniques to optimize the configuration value reasoning using LLM such as dealing numeric value more smartly. We will explain it in our future work. 

\stitle{M13 [Discussion on Generalizability]}:
We will add a discussion in Section 3 to justify that \sys can be easily generalized to other DBMSes, as the algorithms for training data generation, model training, and evaluation are adaptable to new DBMSes. Specifically, when applying \sys to a new DBMS, all that is required is the specification of the knobs and the manuals of the DBMS. \sys can then use these inputs to automatically generate augmented data and train a new model during the offline stage, while supporting evaluation on the DBMS in the online stage.
 % M8 - more detailed experiment analysis
 % (1) Adding recall / precision results
 % (2) Adding statistics information

 % M9 - Including IR literature in related works.
% M10 - clarification on reasoning configuration value
% M11 - clarification on automating training label
 

% \stitle{M2 [New Experiments]}: We will conduct new experiments:
% \begin{enumerate}
%     \item
%     \textbf{More baselines}: For PLM, we will use the same training method of PLM with augmented training data (\textbf{DA + PLM}). For LLM, we will add the following baselines.
%  \textbf{(a) More models:} add more large language models to replace GPT in our existing experiments. Specifically, we use Qwen, Llama-3 to replace GPT with the following baselines - \textbf{Qwen, Llama-3, Qwen (all knobs), Llama-3 (all knobs)}. Moreover, we also replace GPT in \sys as \sys-Qwen, \sys-llama-3. 
% \textbf{(b) Varying prompts}: add more prompt engineers (CoT, task decompose). 
% \textbf{(c) Fine-tuning}: fine-tune GPT 3.5 using the training data.
%  \item \textbf{More retrieval sources}: We will evaluate the overall quality after adding DB statistics from the tables. In particular, we use a template to transfer DB statistics to a text description. Then we add it to \sys's prompt (containing historical questions, manuals and telemetries) and evaluate the reasoning results, comparing it with original \sys.
%  \item \textbf{Time cost quantification}: We will add a user study to evaluate \sys's time cost. Specifically, we will first invite two experienced DBAs to manually solve the problems with provided historical questions, database manuals and telemetries and record the time cost. Second, we will ask two other experts with the same ability to solve the problem using \sys and record the time cost. Finally, we will compare these two records to show how \sys works.

%  \item \textbf{Adding recall / precision results}: We will add recall /precision scores in the NL setting for the overall evaluation.
% \item \textbf{Sensitivity of source quality}: We use the completeness of the included knobs to indicate the quality of the source. We will add a sensitivity experiment to reduce the knobs contained in the source to evaluate the impact of different source quality on \sys performance.

% \item \textbf{Sensitivity of telemetry scale}: We will analyze different scales of telemetry by gradually reducing the metric types and timestamps and evaluate their results.

% \item \textbf{Adding statistics}: We will add more statistics including knob coverage in training questions, historical questions, manuals, and test questions.

% \item \textbf{Dataset}: For the NL setting, we have obtained almost all knob configuration related questions in StackOverflow dataset and MySQL community, it is hard to scale. For the runnable setting, we will add more questions to around 100.

% \end{enumerate}

% \stitle{M3 [Clarifications]}: We will make the following clarifications:

% \begin{enumerate}
%     \item \textbf{Compared with IR literature}: Generally speaking, existing IR algorithms aim to match queries and documents. There are three challenges in the DBMS configuration scenario. 
%     (i) The semantics of documents from different sources may be heterogeneous. For example, historical questions typically describe ``what is wrong'', while DBMS manuals focus on ``How to fix it''. 
%     (ii) For existing IR algorithms, there is a lack of sufficient high-quality training data for DBMS configuration problem. 
%     (iii) It is hard for existing IR algorithms to analyze telemetry data. In general, DBMS configuration requires reasoning and cannot be solved by direct text matching.

%     \item \textbf{Reasoning configuration value}: There are two reasons why LLMs work. 
%     (i) Using RAG, LLM can obtain knowledge about the knobs. For example, LLM can set autocommit=0 with manual "when importing data into InnoDB, turn off autocommit mode, because…", and it can set $innodb\_log\_file\_size=256M$ if the similar question sets the same value. 
%     (ii) LLMs may learn some common settings in pre-training or finetuning phase. Moreover, we agree that we need more techniques to optimize the configuration value reasoning using LLM such as dealing numeric value more smartly. We will explain it in our future work. 

%     \item \textbf{Automating training label}:  The training label can be automated annotated. For the real training data, we use regular expressions to match related knobs from accepted answers or comments of questions. For augmented training data, we generate questions based on a knob’s manual, and this knob is the label corresponding to the questions. We will explain it more clearly in our paper.
% \end{enumerate}


\vspace{-1em}
\section*{Responses to Reviewer \#1}

\begin{shaded}
\noindent\textit{\textbf{R1O1}: Experimental eval should include a few other baselines that use LLMs for solving the same problem\ldots}
\end{shaded}

\noindent\textbf{RESPONSE}: Thanks for the suggestion. To the best of our knowledge, we are the first to develop an LLM-based DBMS diagnosis system designed to accept NL questions on DBMS configuration issues and recommend specific configurations to address the issues. Therefore, to address the concern, we can only add more baselines by replacing the GPT with other LLMs, \eg Qwen and Llama-3. Please refer to \textbf{M2} in our revision plan for details.

\begin{shaded}
\noindent\textit{\textbf{R1O2}: There seems to be a lot of human effort required in collecting ground labels for training and evaluation (including confirmation by experts). Human in the loop in ML requires non-trivial amount of time and dollar cost. More discussion is needed.}
\end{shaded}

\noindent\textbf{RESPONSE}: Sorry for the confusion. We clarify that, actually, \sys does not require much human effort to collect ground labels for training and evaluation due to its automated labeling process. We will revise the experimental setup (Section 6.1) to make it clearer. Please see \textbf{M10} for details. 

\begin{shaded}
\noindent\textit{\textbf{R1O3}: Related to the above point, the goal of \sys is to reduce the time it takes to manually arrive at a solution by expert DBAs. How could the paper quantify this claim?}
\end{shaded}

\noindent\textbf{RESPONSE}: We will add new experiments to evaluate end-to-end time of DBAs to solve issues with / without \sys, so as to qualify how \sys reduce the time. Please see \textbf{M4} for details.
 
\begin{shaded}
\noindent\textit{\textbf{R1O4}: the overall F-1 scores from Table 2 are still not very high for \sys. There seems to be a lot of room for improvement.}
\end{shaded}

\noindent\textbf{RESPONSE}: We first explain why the overall F-1 scores from Table 2 are not very high for \sys. As introduced in Section 6.1, the evaluation in the NL setting requires that \sys's output knobs strictly match the automatically labeled answers, while disregarding other potentially valid knobs. This can lead to an underestimation of the F1-score, which is why we proposed the Runnable setting. In the Runnable setting, DBMS experts assess whether the recommended configurations resolve the issues. As shown in Table 2, \sys achieves a SuccessRate of over 0.7.

Moreover, we agree that ``there seems to be a lot of room for improvement'' -- we really hope for a call-to-arms to significantly push this core database problem. To support this effort, we will conduct an in-depth analysis of the bad cases produced by \sys. Please refer to \textbf{M1} for more details.

%In the NL setting, it requires that the output knobs must be strictly the same as the answer, while ignoring some other knobs that may be valid. This is the reason for the low F1-score and why we propose the Runnable setting. To show this, we will add case studies for bad cases. Please see \textbf{M1} for details. We agree that ``there seems to be a lot of room for improvement'' -- we really hope for a call-to-arms 
%to significantly push this core database problem.

\begin{shaded}
\noindent\textit{\textbf{R1O5}: What was the actual prompt submitted to the LLM? It wasn't presented in the main body of the paper.}
\end{shaded}

\noindent\textbf{RESPONSE}: 
Please refer to Figure 2(b) as an illustrative prompt submitted to the LLM. To make it clearer, we will add more real prompts in experiments in case studies (see \textbf{M1}). Moreover, we have already included all the prompts in our experiments in the repo: 
\url{https://anonymous.4open.science/r/Andromeda-D150/}

\begin{shaded}
\noindent\textit{\textbf{R1O6}: it would also be particularly insightful to discuss some loss cases for \sys for which it does not do well and how \sys could be improved to address those loses?}
\end{shaded}

\noindent\textbf{RESPONSE}: We will include a detailed analysis of the bad cases to highlight the limitations of \sys and discuss potential improvements. Please refer to \textbf{M1} for more details.

\begin{shaded}
\noindent\textit{\textbf{R1O7}: How generalizable is \sys to other DBMSes? Would it required training data generation, model training, and evaluation for each DBMS?}
\end{shaded}

\noindent\textbf{RESPONSE}: 
\sys can be easily generalized to other DBMSes. Please see \textbf{M13} for more details. 
% it needs to regenerate augmented data and retrain a new model in the offline stage because different DBMSs contain different knobs and manuals. Nevertheless, the algorithms for DA and training can be generalized.

\begin{shaded}
\noindent\textit{\textbf{R1O8}: The paper talks about the time efficiency of \sys but a discussion on the cost efficiency is missing.}
\end{shaded}

\noindent\textbf{RESPONSE}: As suggested, we will report the cost efficiency, which is the average cost of calling LLMs for each NL debugging question $q$. Please see \textbf{M8} for more details. 

%Thanks for the suggestion. To calculate the cost of each query, we have calculated the average cost of prompt and response respectively and we add the prompt cost and response cost as the cost efficiency. In detail, 
%\begin{itemize}
%    \item GPT-3.5 costs $0.0017$\$ / query. 
%    \item GPT-4 costs $0.053$\$ / query. 
%    \item GPT-3.5 (all knobs) costs $0.012$\$ / query. 
%    \item GPT-4 (all knobs) costs $0.039$\$ / query.
%    \item \sys-3.5 costs $0.006$\$ / query.
%    \item \sys 4 costs $0.022$\$ / query.
%\end{itemize}

%We will add a more detailed report on the cost efficiency in experiments.

\stitle{Minor Remarks:}

\begin{shaded}
\noindent\textit{\textbf{R1C1}: It appears all telemetry data is always analyzed in real-time? There seems to be a lot of room for optimization here. %Please comment.
}
\end{shaded}

\noindent\textbf{RESPONSE}: 
Yes, the telemetry data is analyzed in real-time. We have conducted a latency analysis, as reported in Table 8. The result shows that the time used for telemetry analysis is 2.85 seconds, which we believe is acceptable for users. 
However, we agree that there is room for optimization, such as filtering out unnecessary telemetry data. We will address this in future work.

%Yes, the telemetry data is analyzed in real-time. Actually, we have conducted the latency analysis in Table 8. The time consumption is in seconds, which we think is acceptable to users. In addition, we agree that there exists room for optimization, such as filtering useless telemetry. We will add it in our future work.

\begin{shaded}
\noindent\textit{\textbf{R1C2}: How does \sys (and related approaches) deal with cases where a small variation of a question compared to a historical question leads to a very different solution?}
\end{shaded}

\noindent\textbf{RESPONSE}: 
\sys deals with these cases by matching domain-specific contexts from other sources, including troubleshooting manuals and DBMS telemetry data. This is one of the key reasons we use multiple sources in our RAG approach. Specifically, when relying solely on historical questions is not sufficient, prioritizing relevant manuals or telemetry data over potentially confusing historical questions can provide more accurate solutions.


%\sys addresses these cases by matching domain-specific contexts for the question from other sources, including troubleshooting manuals and DBMS telemetries. Actually, this is the key reason that motivates us to use multiple sources for RAG. Specifically, when using single historical questions as sources is not helpful, ranking the helpful manuals/telemetries before this confusing historical question may help.

%For those cases where a small variation of a question compared to a historical question leads to a very different solution, using single historical questions as sources is not helpful. To deal with it, \sys uses multiple sources for RAG, for example, ranking the helpful manuals before this confusing historical question can help.

\begin{shaded}
\noindent\textit{\textbf{R1C3}: there could be multiple ways to fix the same issue? It's unclear how \sys and related approaches are reasoning about and ranking between different tuning knobs?}
\end{shaded}

\noindent\textbf{RESPONSE}: Yes, there could be multiple ways, such as different tuning knobs, to fix the same issue, as illustrated in Figure 2(b). \sys uses an LLM to reason about the various tuning knobs and selects the most appropriate set. Please see \textbf{M12} for details. 

%Specifically, as discussed in \emph{Step 3} of the online stage in Section 3, \sys generates a prompt that includes all the retrieved data and then calls the LLM to recommend the configurations, i.e., the tuning knobs, to address the issue. We will revise Section 3 to clarify this further.

%
%Yes, there could exist multiple ways, \ie tuning knobs, to fix the same issue, as shown in Figure 2(b). \sys relies on an LLM to reason about between different tuning knobs and identify an appropriate set of knobs. Specifically, as discussed in \emph{Step 3} in the online stage of Section 3, \sys generates an prompt by including all the retrieved data and calls an LLM to generate the configuration recommendations, \ie tuning knobs, to fix the issue. We will revise Section 3 to make it clearer. 

%
%For the reasoning of \sys, it outputs the most related knobs using LLM to select knobs from candidate knobs in multi-sources as the top-1 result for the query. 

\begin{shaded}
\noindent\textit{\textbf{R1C4}: %In Sec 4.3, it's unclear by 
	why manual-manual samples are prioritized over others?}
\end{shaded}

\noindent\textbf{RESPONSE}: 
We conducted an experiment to evaluate different prioritization strategies, and the results show that prioritizing manual-manual training samples yields the best performance. The primary reason is that aligning manual-manual samples is ``easier'' than aligning question-question or manual-question samples due to the formality and consistency of manuals. By training our Alignment component on these easier cases first, we ensure it is well-prepared before gradually improving it on more challenging cases.
%
%We conducted an empirical evaluation of various configurations and found that prioritizing manual-manual samples yields the best quality. Our analysis suggests that optimizing models individually first benefits joint training. Specifically, optimizing the manual embedding model with manual-manual samples and the question embedding model with question-question samples leads to better performance when training multiple models using question-manual samples.
% Manual-manual samples are prioritized over others, because training manual-manual samples is the basis for training question-manual / manual-question samples. Given a question, the target of training manual-manual samples is to correctly represent manuals in hidden space to deal with multi-source heterogeneity. And after manuals currently embedded, \sys should learn to adjust question and manual embeddings based on the trained manual embeddings. 


\begin{shaded}
\noindent\textit{\textbf{R1C5}: %The document embeddings are stored in a vector DB. May be some quick mention of 
	what kind of vector DB and what kind of and size of indexes are needed to meet the runtime SLA of \sys?}
\end{shaded}

\noindent\textbf{RESPONSE}: We use Meta Faiss as our vector database to index the embeddings of historical questions and manuals. In the current implementation of \sys, we have indexed 5,138 vectors for MySQL and 1,158 vectors for PostgreSQL, with each vector having a dimension of 768. We will provide further clarification on this further in the paper.

\begin{shaded}
\noindent\textit{\textbf{R1C6}: Analyzing a large amount of telemetry data and zooming in on the sections that might be correlated with the issue being debugged does not seem to be a new challenge and there may already be existing approaches.}
\end{shaded}

\noindent\textbf{RESPONSE}: 
There are two key challenges that distinguish our work. First, detecting anomalous telemetry data from vast amounts of time-series information is particularly difficult due to the influence of seasonality and trends, which can obscure what is truly anomalous. Second, existing approaches do not address the semantic correlation between natural language queries and telemetry data, which is an essential aspect of our solution.
% There are two new challenges: The first challenge is detecting anomalous telemetries from a huge amount of time-series data, as it is not easy to identify what is anomalous with the influence of sessonal and trand. Secondly, existing works do not consider the sematic correlation of the NL query and telemetries.
% We are the first to deal with user database diagnosis text questions using telemetry data. In detail, existing works analyze telemetry through only one aspect (such as the d-bot use rule to detect anomaly in telemetry). In contrast, our work comprehensively analyzes telemetry from multiple aspects that are anomalies in time series data of metric, the correlation of query and metrics with the description of metrics in manual. 

%
%\begin{shaded}
%\noindent\textit{\textbf{Required Changes}: O1, O2, O4, O6, %O8 (and addressing minor comments)}
%\end{shaded}
%
%\noindent\textbf{RESPONSE}: We have addressed all concerns. %Please see our responses mentioned above.
\vspace{-1em}
\section*{Responses to Reviewer \#2}

\begin{shaded}
\noindent\textit{\textbf{R2O1}: The experimental setup and findings lack sufficient details \ldots
	 %to aid understanding. For example, 
	 (1) the paper should explore which types of queries LLMs perform well on, where RAG helps, and whether historical queries can be categorized by type and frequency. It should also examine how the system performs for queries with less frequent questions. 
	 %
	 (2)Including results on precision and recall in Table 2 would also help.}
\end{shaded}

\noindent\textbf{RESPONSE}: 
Thank you for the suggestion. We will revise the paper by providing more details about experimental setup and findings.

(1) We have already categorized queries by considering the frequency and types of their ground-truth labels (i.e., the tuning knobs). Specifically, as shown in Figures 7 and 8, we classify queries into high-, medium-, and low-frequency categories. We have also explored the questions raised by the reviewer. For instance, in most cases, LLMs perform better on high-frequency queries compared with medium- and low-frequency ones, while RAG consistently improves performance across all frequency levels. Additionally, we have examined \sys's performance on less frequent queries. In Figure 9, we further categorize queries by the type of their corresponding knobs (i.e., numerical, categorical, and boolean). Our findings show that \sys achieves better performance on numerical and boolean queries compared to categorical ones. 

(2) As suggested, we will include precision and recall results in Table 2 to make the comparison more comprehensive.

We will revise the paper to include detailed explanations of these experimental findings, as indicated in \textbf{M9}. 

%Thanks for the suggestions. As discussed in \textbf{M1}, We have conducted sensitivity experiments of the type of knob in different queries and the frequency of the knob in the queries in Figure 7, Figure 8 and Figure 9. If more sensitivity experiments are needed, we can add them when revising the paper. Moreover, we will conduct case studies (see \textbf{M1})to show which queries are successfully solved and which are failed in analyzing the reasons. And we will add recall / precision in Table 2.

\begin{shaded}
\noindent\textit{\textbf{R2O2}: Traditional IR techniques have long addressed issues of query-document matching, but the paper does not discuss these prior works in detail. The paper should highlight the unique challenges in DBMS configuration debugging that necessitate novel approaches.}
\end{shaded}

\noindent\textbf{RESPONSE}:
%The unique challenge is that historical questions and DBMS manuals are from different sources, where the semantics may be heterogeneous. 
As suggested, we will revise the Related Work section to include a detailed discussion of traditional IR techniques and highlight the unique challenges. Please see \textbf{M11} for details. 

%To clarify, compared to traditional IR approaches, the unique challenge here lies in retrieving documents from multiple sources, such as historical questions and DBMS manuals, where the semantics of documents from different sources may be heterogeneous. For instance, as illustrated in Figure 2, historical questions typically describe ``what is wrong'' (\eg ``\emph{It takes over 15 minutes\ldots}''), while DBMS manuals focus on ``how to fix it'' (\eg ``\emph{turn off autocommit mode}''). We will expand on this point in the revised Related Work section.
%
%
%Thank you for the suggestion. We will revise the Related Work section to include traditional IR techniques in detail. 
%
%We clarify that, compared with such traditional IR techniques, the unique challenge is that retrieving documents from multiple sources, such as historical questions and DBMS manuals, where the semantics of documents from different sources may be heterogeneous. For example, as shown in Figure 2, historical questions typically describe ``what is wrong'' (e.g., ``It takes over 15 minutes . . .''), while DBMS manuals focus on ``How to fix it'' (e.g., ``turn off autocommit mode'').
%We will discuss this in more detail in the Related Work. 
%
%Please see \textbf{M3 (1)} for details.


\begin{shaded}
\noindent\textit{\textbf{R2O3}: %The effectiveness of the approach heavily relies on the quality and relevance of historical questions, troubleshooting manuals, and telemetry data. 
	(1) Inaccuracies in these sources could lead to incorrect or suboptimal debugging suggestions. 
	(2) Achieving high accuracy in document retrieval among such diverse data types is inherently challenging and can affect overall performance. 
	The paper should discuss (if possible empirically) the sensitivity of the approach to these factors.
}
\end{shaded}

\noindent\textbf{RESPONSE}: Thanks for pinpointing these crucial factors.

(1) We agree that inaccuracies in sources of historical questions, troubleshooting manuals and telemetries can significantly impact overall performance. As suggested, we will add new experiments to empirically investigate these factors. 
%For instance, we plan to introduce noise into the ground-truth labels of historical questions and troubleshooting manuals to evaluate the sensitivity of our approach. 
Please see \textbf{M5} for details. 

(2) We have already explored the impact of document retrieval on overall performance in Section 6.3. Our results show that the effectiveness of document retrieval significantly affects the overall performance. For example, our proposed retrieval method, which combines different types of documents, not only achieves better retrieval performance (i.e., higher recall) but also enhances overall results compared to using a single type of document.
%, as shown in Figures 7 and 8. 

%We will add a more detailed analysis in this section.

%Thanks for the suggestions. We agree that the effectiveness of the approach heavily relies on the quality and relevance of historical questions, troubleshooting manuals, and telemetry data. To show this point, we will add an experiment to discuss the sensitivity by adjusting the completeness of sources. More details can be referred to \textbf{M2 (5)}. 

\begin{shaded}
\noindent\textit{\textbf{R2O4}: %Analyzing telemetry data involves understanding a wide array of metrics, which can be complex and slow. 
	(1) The paper should provide more details on the scalability of the approach (both in number and types) for detecting relevant telemetries. (2) it should address whether telemetries are "always" necessary, what queries benefit more telemetries, and what happens when there is ambiguity.}
\end{shaded}

\noindent\textbf{RESPONSE}: (1) As suggested, we will add a new experiment to examine the scalability of our approach for detecting relevant telemetry data. Specifically, we will vary the number of input metrics and differentiate between metric types, and report the time required for telemetry data analysis. 
Please refer to \textbf{M6}. 

(2) We have already analyzed the impact of telemetry data in Section 6.4. Our experimental results suggest that telemetry data may not ``always'' be necessary, as shown in Figure 9. Specifically, compared to \sys-docs-only (i.e., without telemetry data), \sys does not always demonstrate superior performance. This is because some anomalies are not caused by anomalous resource usage, such as the error ``\emph{column `DateReceived' cannot be null}'' shown in Figure 1. Additionally, we found that queries involving tuning numerical knobs tend to benefit more from telemetry data. We will revise Section 6.4 to provide a more detailed analysis.


%We will add a telemetry scale sensitivity experiment to analyze the impact of telemetry data size on running time. Please see \textbf{M2 (6)} for details. Actually, the telemetries may not ``always'' be necessary because some anomalies are not caused by the anomalous resources usage, such as the error ``The column `DateRecieved' cannot be null'' in Figure 1, and we have discussed it in Exp-4 in detail.

\begin{shaded}
\noindent\textit{\textbf{R2O5}: %Overall, the results appear to be on the lower end (with F1 score over < 0.50). 
	The paper should explain why these results are statistically significant (e.g, how does it significantly reduces the operational burden) compared to the option of having a DBA search discussion or community forums. 
	Furthermore, %it might help to 
 discuss how the provided results by \sys can be trusted w/o significant troubleshooting.}
\end{shaded}

\noindent\textbf{RESPONSE}:
We will conduct a new experiment to evaluate whether \sys offers a statistically significant advantage over DBAs searching through discussion or community forums
%
%evaluate the time taken by DBAs to solve problems with and without \sys, in order to determine whether \sys offers a statistically significant advantage over DBAs searching through discussion or community forums. 
Please see \textbf{M4} for details.

We will add a discussion in Section 3 on how \sys can be trusted. The key idea is that \sys not only provides configuration recommendations but also offers \emph{explanations}, grounded in historical questions, troubleshooting manuals, and telemetry data. 
%We will also revise Figure 2 to illustrate the explanations. 

%In the NL setting, it requires that the output knobs must be strictly the same as the answer, while ignoring some other knobs that may be valid. This is the reason for the low F1-score and why we propose the Runnable setting. To explain why these results are statistically significant, we add an experiment to quantify the time cost of DBA to solve problems (see \textbf{M2 (3)}). Moreover, we will add case studies to our experiments to show how \sys works and the improvement room. Please see M1 for details.

%
%\stitle{Required Changes: }
%
%\begin{shaded}
%\noindent\textit{\textbf{R2C1}: Dig more into the details on %experiments \ldots% to help understand the result. Please 01.
%}
%\end{shaded}
%
%\noindent\textbf{RESPONSE}: %We will add more experiments %and discussion about our results (
%Please see our responses to \textbf{R2O1}.
%
%\begin{shaded}
%\noindent\textit{\textbf{R2C2}: Provide more details on how %the approach scales in capturing telemetry %data/characteristics. %Please 04.
%}
%\end{shaded}
%
%\noindent\textbf{RESPONSE}: %We will add a telemetry scale sensitivity experiment to analyze the impact of telemetry data size on running time. 
%Please see our responses to \textbf{R2O4}.

%\begin{shaded}
%\noindent\textit{\textbf{R2C3}: Briefly compare and constrast with existing body of research query-document matching, highlighting characteristics of problem that necessisates a new approach the paper proposes. %Please see O2.
%}
%\end{shaded}

%\noindent\textbf{RESPONSE}: %We will discuss it more clearly in the related work of our paper. 
%Please see our responses to \textbf{R2O2}. 

%\begin{shaded}
%\noindent\textit{\textbf{R2C4}: Not a must but also see if O3 and P5.}
%\end{shaded}
%
%\noindent\textbf{RESPONSE}: %We will address these concerns as 
%Please see our responses to \textbf{R2O3} and \textbf{R2O5}. 

\vspace{-1em}
\section*{Responses to Reviewer \#3}

\begin{shaded}
\noindent\textit{\textbf{R3O1}: %While it make sense that LLMs can help identify relevant configuration knobs, 
the intuition why it is a good candidate for recommending knob values is not as clear. LLMs are not particularly good at numerics. I wonder why the problem setup chooses to directly output the knob value, instead of suggesting directional adjustments (e.g., increase/decrease, enable/disable).}
\end{shaded}

\noindent\textbf{RESPONSE}: 
We will include a detailed discussion in Section 3 to justify the intuition why LLM is good for recommending knob values. Please see \textbf{M12} for details. 
%
The reason why we directly output the knob value is that it is more convenient for the user to set an exact value than suggesting directional adjustments. For example, if \sys recommends the user to increase a knob, user may still not know which value is suitable. 

%We agree that LLMs are not particularly good at numerics because the value setting depends on the runnable environment and cannot be solved simply by LLM using documentation or experience. As a result, there exists more optimization. We will explain it clearer in our future work. 

%

\begin{shaded}
\noindent\textit{\textbf{R3O2}: %In addition to telemetry data, 
it seems like statistics on the sql table, statistics of query workload and machine resources such as memory size could also play a role in debugging. 
%For example, physical memory of the machine could affect knob choices such as buffer pool or table size.
}
\end{shaded}

\noindent\textbf{RESPONSE}: 
%We agree that these statistics play a role in debugging. 
We will conduct new experiments to evaluate the impact of these statistics. 
Please see \textbf{M7} for details.

%
%As some statistics (query workload and machine resources are included in telemetry), we will add DB statistics from the tables as a new source for \sys in the experiment to verify this claim. Please see \textbf{M2 (2)} for details.

\begin{shaded}
\noindent\textit{\textbf{R3O3}: %With only a few hundred training data points, it’s unsurprising that the PLM baseline shows very poor performance. 
This PLM baseline could be made stronger if you augment the training data using examples generated from Section 4.2.}
\end{shaded}

\noindent\textbf{RESPONSE}: We will add this baseline in the revised version, as described in \textbf{M2}.

%augment the training data for PLM as a new baseline. Please see \textbf{M2 (1)} for more details.

\begin{shaded}
\noindent\textit{\textbf{R3O4}: It would also help to get some idea on the coverage of the evaluation datasets. What percent of MySQL/Postgres knobs were covered in the documentation, manual and test datasets?}
\end{shaded}

\noindent\textbf{RESPONSE}: 
%Thanks for the suggestions. 
We will discuss this further, as described in \textbf{M9}.

%add these statistics (knob coverage in training questions, historical questions, manuals and test questions) in our experiments. Please see \textbf{M2 (7)}.

\stitle{Minor remarks}:

\begin{shaded}
\noindent\textit{\textbf{R3C1}: Numeric knobs have higher success rate than categorical ones (Figure 9). Does it mean that the specific values of numeric knobs do not matter that much - multiple values would work.}
\end{shaded}

\noindent\textbf{RESPONSE}: Yes, multiple values would work. %In many cases, correctly choosing to lower/raise the knob value may solve the user's questions. 
We will explain this in the case study (see \textbf{M1}).

% \vspace{-1em}
\begin{shaded}
\noindent\textit{\textbf{R3C2}: It wasn’t clear until the evaluation that there are essentially two version of \sys. One is only concerned with identifying the correct subset of the knobs and does not predict knob values (the NL setting). The other takes telemetry data and also predicts knob values (the Runnable setting).}
\end{shaded}

\noindent\textbf{RESPONSE}: Thanks. We will clarify it when introducing the framework in Section 3.

\begin{shaded}
\noindent\textit{\textbf{R3C3}: In section 6.4 “ (2) \sys-telemetry-only: \sys without telemetry data analysis, (3) \sys- docs-only: \sys without document retrieval”. Is this a typo? 
%Does “\sys-telemetry-only” mean \sys with telemetry data analysis?
}
\end{shaded}

\noindent\textbf{RESPONSE}: We will fix it. Thanks!

%
%\begin{shaded}
%\noindent\textit{\textbf{Required Changes}: O1-O4}
%\end{shaded}
%
%\noindent\textbf{RESPONSE}: We will address all concerns in %O1-O4.
%

% \vspace{-1em}
\section*{Responses to Meta Reviewer}
 
\begin{shaded}
\noindent\textit{\textbf{C1}: (1)The reviewers felt the experiments warranted more specific motivations — characterizing the types of queries for which these techniques are (and are not) effective, and assessing the sensitivity of these methods to question frequency in the training data. (2) Providing experiments to show more specifically where the proposed approach does or does not excel would provide a more nuanced recommendation for practitioners — some results are modest, and limitations are not discussed.}
\end{shaded}

\noindent\textbf{RESPONSE}:
(1) Please refer to our responses to \textbf{R2O1}. (2) See our responses to \textbf{R1O4} and \textbf{R2O5}.
% As discussed in \textbf{R2O1}, we have conducted a sensitivity analysis in Figure 7, Figure 8 and Figure 9. And we will add more case studies (see \textbf{M1}) in our experiments to show why \sys works and what is the room to improve.

\begin{shaded}
\noindent\textit{\textbf{C2}: (1) The reviewers also noted that the experiments are limited to a small dataset, which puts competitive methods at a disadvantage. If this limited dataset is realistic, some additional motivation is warranted. Otherwise, increasing its size to provide a more realistic setting for competitive methods would make the argument more convincing. (2) A related issue is the availability of training labels — the cost in time and training warrants additional discussion. (3) In addition, providing more baselines involving LLMs (e.g., varying prompting, fine-tuning, or other setups). Your shepherd can assist with considering additional experiments and discussion.}
\end{shaded}

\noindent\textbf{RESPONSE}: 
(1) We will increase the dataset size. Please refer to \textbf{M3}. (2) Please refer to our responses to \textbf{R1O2}. (3) We will add these baselines in the experiments. Please refer to \textbf{M2}.
%We will increase the size of the dataset in the Runnable setting. Please see details in \textbf{M2 (8)}. For the availability of training labels, the labeling process is automated and does not cost much time. Please see \textbf{M3 (3)} for details. We will clarify this in our paper. In addition, we will add more baselines as we discussed in \textbf{M2 (1)}.

\begin{shaded}
\noindent\textit{\textbf{C3}: (1) There was also consensus that the paper could be significantly improved by highlighting the unique challenges in this context of configuration debugging relative to more general query-document matching in the IR literature, and (2) the generalizability of the system to other DBMS. (3) Also, some design decisions warrant more discussion: The output is numeric settings, but LLMs can struggle with reasoning about numeric values. Therefore some discussion about alternatives, including qualitative adjustments (direction, categorical magnitudes) could produce different results.}
\end{shaded}

\noindent\textbf{RESPONSE}: 
(1) Please refer to our responses to \textbf{R2O2}. (2) Please refer to our responses to \textbf{R1O7} or \textbf{M13}. (3) Please refer to our responses to \textbf{R3O1} or \textbf{M12}.

% As we discussed in \textbf{M3 (1)} and \textbf{R2O2}, the unique challenge is that historical questions and DBMS manuals are from different sources, where the semantics may be heterogeneous. We will discuss it more clearly in related work. For design decisions, as we discussed in \textbf{M3 (2)} and \textbf{R3O1}, compared with qualitative adjustments, directly setting knob value can be more convenient for users and LLM can accomplish value setting by leveraging in-context knowledge and trained knowledge to decide the value. Moreover, we agree that these methods have room for improvement for numeric values, which we will clarify in our future work.

\begin{shaded}
\noindent\textit{\textbf{C4}: %The reviewers felt 
\ldots the results could be improved by providing additional contextual information to the LLM: machine resources, DB statistics from the tables, statistics of the query workload when available. %Some discussion or additional experiments of these effects would help show new directions.
}
\end{shaded}

\noindent\textbf{RESPONSE}:
Please refer to our responses to \textbf{R3O2}
% As discussed in \textbf{M2 (2)} and \textbf{R3O2}, we will add DB statistics from the tables as a new source for \sys in the experiment and discuss the results.  


\begin{shaded}
\noindent\textit{\textbf{Required Changes}: Overall: R1O1, R1O2, R1O4, R1O7, R2O1, R2O2, R2O4, R3O1, R3O3; Optional changes include R103, R1O5, R1O6, R1O8, R2O3, R3O2}
\end{shaded}

\noindent\textbf{RESPONSE}: We will address all the concerns.




==> tables/augment_reasoning_1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}
\caption{Reasoning result of different augmentation methods.}
\begin{tabular}{|c|cccccccc||cc|}
\hline
Evaluation types & \multicolumn{8}{c||}{Text questions only (F1-score)}                                                                                                                                                                                                                                                     & \multicolumn{2}{c|}{Workload (Accuracy)}             \\ \hline
Datasets      & \multicolumn{2}{c|}{MySQL SO}                                             & \multicolumn{2}{c|}{MySQL Forum}                                          & \multicolumn{2}{c|}{PG SO}                                                & \multicolumn{2}{c||}{Runnable-Q}                        & \multicolumn{2}{c|}{Runnable-Q}                        \\ \hline
LLM models    & \multicolumn{1}{c|}{GPT-3.5}        & \multicolumn{1}{c|}{GPT-4}          & \multicolumn{1}{c|}{GPT-3.5}        & \multicolumn{1}{c|}{GPT-4}          & \multicolumn{1}{c|}{GPT-3.5}        & \multicolumn{1}{c|}{GPT-4}          & \multicolumn{1}{c|}{GPT-3.5}        & GPT-4          & \multicolumn{1}{c|}{GPT-3.5}        & GPT-4          \\ \hline
No Augment    & \multicolumn{1}{c|}{0.306}          & \multicolumn{1}{c|}{0.37}           & \multicolumn{1}{c|}{0.317}          & \multicolumn{1}{c|}{0.411}          & \multicolumn{1}{c|}{0.287}          & \multicolumn{1}{c|}{0.336}          & \multicolumn{1}{c|}{0.319}          & 0.41           & \multicolumn{1}{c|}{0.529}          & 0.627          \\ \hline
CoT Augment   & \multicolumn{1}{c|}{0.32}           & \multicolumn{1}{c|}{0.378}          & \multicolumn{1}{c|}{0.328}          & \multicolumn{1}{c|}{0.406}          & \multicolumn{1}{c|}{0.331}          & \multicolumn{1}{c|}{0.348}          & \multicolumn{1}{c|}{0.365}          & 0.394          & \multicolumn{1}{c|}{0.647}          & 0.686          \\ \hline
\sys-docs-only           & \multicolumn{1}{c|}{\textbf{0.352}} & \multicolumn{1}{c|}{\textbf{0.402}} & \multicolumn{1}{c|}{\textbf{0.379}} & \multicolumn{1}{c|}{\textbf{0.417}} & \multicolumn{1}{c|}{\textbf{0.352}} & \multicolumn{1}{c|}{\textbf{0.411}} & \multicolumn{1}{c|}{\textbf{0.428}} & \textbf{0.505} & \multicolumn{1}{c|}{\textbf{0.725}} & \textbf{0.765} \\ \hline
\end{tabular}
\label{tab:augment_reasoning}
\end{table*}

==> tables/overall.tex <==
\begin{table*}
\caption{Overall quality comparasion.}
\begin{tabular}{|c|cccc||c|}
\hline
      Evaluation type                  & \multicolumn{4}{c||}{Text questions only (F1-score)}                                                       & Workloads (Accuracy) \\ \hline
corpus                    & \multicolumn{1}{c|}{MySQL SO}          & \multicolumn{1}{c|}{MySQL Forum}          & \multicolumn{1}{c|}{PG SO}             & Runnable-Q & Runnable-Q               \\ \hline
PLM                       & \multicolumn{1}{c|}{0.018}             & \multicolumn{1}{c|}{0.004}                & \multicolumn{1}{c|}{0.006}             & 0.004          &    -                  \\ \hline
GPT 3.5                   & \multicolumn{1}{c|}{0.221}             & \multicolumn{1}{c|}{0.07}                & \multicolumn{1}{c|}{0.201}               & 0.244          &    0.490                  \\ \hline
GPT 4                     & \multicolumn{1}{c|}{0.222}             & \multicolumn{1}{c|}{0.05}                & \multicolumn{1}{c|}{0.161}             & 0.339          &     0.471                \\ \hline
GPT 3.5 (all knobs)       & \multicolumn{1}{c|}{0.308}             & \multicolumn{1}{c|}{0.269}                & \multicolumn{1}{c|}{0.299}             &  0.359         &   0.510                   \\ \hline
GPT 4  (all knobs)        & \multicolumn{1}{c|}{0.332}             & \multicolumn{1}{c|}{0.253}                & \multicolumn{1}{c|}{0.390}             & 0.478          &     0.569               \\ \hline
\sys-gpt-3.5              & \multicolumn{1}{c|}{0.348}             & \multicolumn{1}{c|}{0.382}                & \multicolumn{1}{c|}{0.321}             & 0.424          &  \textbf{0.765}              \\ \hline
\sys-gpt-4                & \multicolumn{1}{c|}{\textbf{0.441}}    & \multicolumn{1}{c|}{\textbf{0.449}}       & \multicolumn{1}{c|}{\textbf{0.398}}    & \textbf{0.506} &   0.706        \\ \hline
\end{tabular}
\label{tab:overall}
\end{table*} 

==> tables/overall_1.tex <==
\begin{table*}
\caption{Overall quality comparasion.}
\begin{tabular}{|c|cccc||c|}
\hline
      Evaluation type                  & \multicolumn{4}{c||}{Text questions only (F1-score)}                                                       & Workloads (Accuracy) \\ \hline
corpus                    & \multicolumn{1}{c|}{MySQL SO} & \multicolumn{1}{c|}{MySQL Forum} & \multicolumn{1}{c|}{PG SO} & Runnable-Q & Runnable-Q               \\ \hline
PLM                         & \multicolumn{1}{c|}{0.018}    & \multicolumn{1}{c|}{0.004}       & \multicolumn{1}{c|}{0.006}    & 0.004 &    -                  \\ \hline
GPT 3.5                     & \multicolumn{1}{c|}{0.225}    & \multicolumn{1}{c|}{0.168}       & \multicolumn{1}{c|}{0.2}    & 0.159   &    0.275                  \\ \hline
GPT 4                       & \multicolumn{1}{c|}{0.204}    & \multicolumn{1}{c|}{0.112}       & \multicolumn{1}{c|}{0.137}    & 0.146 &     0.216                \\ \hline
GPT 3.5 (all knobs)                & \multicolumn{1}{c|}{0.291}    & \multicolumn{1}{c|}{0.234}       & \multicolumn{1}{c|}{0.3.4}    &  0.216  &   0.392                   \\ \hline
GPT 4  (all knobs)                    & \multicolumn{1}{c|}{0.311}    & \multicolumn{1}{c|}{0.314}       & \multicolumn{1}{c|}{0.299}    & 0.406 &     0.647               \\ \hline
\sys-gpt-3.5 & \multicolumn{1}{c|}{0.352}    & \multicolumn{1}{c|}{0.379}       & \multicolumn{1}{c|}{0.352}    & 0.454 &          \textbf{0.804}              \\ \hline
\sys-gpt-4   & \multicolumn{1}{c|}{\textbf{0.402}}    & \multicolumn{1}{c|}{\textbf{0.426}}       & \multicolumn{1}{c|}{\textbf{0.398}}    & \textbf{0.539} &             0.784        \\ \hline
\end{tabular}
\label{tab:overall}
\end{table*} 

==> tables/overall_runnable.tex <==
\begin{table}[]
\caption{Overall Accuracy on ``Runnable cases'' .}
\begin{tabular}{|c|cc|}
\hline
Datasets        & \multicolumn{2}{c|}{Runnable cases}                  \\ \hline
LLM models      & \multicolumn{1}{c|}{GPT-3.5}        & GPT-4          \\ \hline
GPT             & \multicolumn{1}{c|}{0.490}          & 0.471          \\ \hline
GPT (all knobs) & \multicolumn{1}{c|}{0.510}          & 0.569          \\ \hline
sys             & \multicolumn{1}{c|}{\textbf{0.765}} & \textbf{0.706} \\ \hline
\end{tabular}
\label{tab:overall_runnable}
\end{table}

==> tables/overall_text.tex <==
% \begin{table}[]
% \caption{Overall F1-scores on ``NL questions only'' .}

%  \resizebox{\columnwidth}{!}{
% \begin{tabular}{|c|cl|cl|cl|}
% \hline
% \quad\, \textbf{Datasets} \quad\,  & \multicolumn{2}{c|}{\,\, \,\,  \textbf{MySQL SO} \quad\,} & \multicolumn{2}{c|}{\,\,   \textbf{MySQL Forum} \, } & \multicolumn{2}{c|}{\quad\, \, \,\,   \textbf{PG SO} \quad\quad\quad} \\ \hline
% PLM  & \multicolumn{2}{c|}{0.018}    & \multicolumn{2}{c|}{0.004}       & \multicolumn{2}{c|}{0.006} \\ \hline
% \end{tabular}
% }

% \vspace{0.3em}
%  \resizebox{1\columnwidth}{!}{
% \begin{tabular}{|c|cc|cc|cc|}
% \hline
% \textbf{Datasets}        & \multicolumn{2}{c|}{\textbf{MySQL SO}}                        & \multicolumn{2}{c|}{\textbf{MySQL Forum}}                     & \multicolumn{2}{c|}{\textbf{PG SO}}                           \\ \hline
% \textbf{LLM models}      & \multicolumn{1}{c|}{\textbf{GPT-3.5}}        & \textbf{GPT-4}          & \multicolumn{1}{c|}{\textbf{GPT-3.5}}        & \textbf{GPT-4}         & \multicolumn{1}{c|}{\textbf{GPT-3.5}}        & \textbf{GPT-4}          \\ \hline
% GPT             & \multicolumn{1}{c|}{0.221}          & 0.222          & \multicolumn{1}{c|}{0.07}           & 0.05           & \multicolumn{1}{c|}{0.201}          & 0.339          \\ \hline
% GPT (all knobs) & \multicolumn{1}{c|}{0.308}          & 0.332          & \multicolumn{1}{c|}{0.269}          & 0.253          & \multicolumn{1}{c|}{0.299}          & 0.390          \\ \hline
% sys             & \multicolumn{1}{c|}{\textbf{0.348}} & \textbf{0.441} & \multicolumn{1}{c|}{\textbf{0.382}} & \textbf{0.449} & \multicolumn{1}{c|}{\textbf{0.321}} & \textbf{0.398} \\ \hline
% \end{tabular}
% }
% \label{tab:overall_text}
% \end{table}


\begin{table*}
\caption{Overall results, where we measure F1-score in the NL setting, and SuccessRate in the Runnable setting. 
	%As PLM predicts too many knobs (over $100$), it is difficult for human to tune these knobs, so we do not evaluate it on MySQL Run.
 } 
\label{tab:overall}
\vspace{-1em}
 \resizebox{0.95\textwidth}{!}{
\begin{tabular}{|c|c||c|c|c|c|c|c|c|}
\hline
\textbf{Datasets} & \textbf{Metrics} & \textbf{PLM} & \textbf{GPT-3.5} & \textbf{GPT-4} & \textbf{\begin{tabular}[c]{@{}c@{}}GPT-3.5 \\ (all knobs)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}GPT-4\\  (all knobs)\end{tabular}} & \textbf{\sys-GPT 3.5} & \textbf{\sys-GPT 4} \\ \hline \hline
MySQL SO          & F1-score              & 0.018        & 0.221            & 0.222          & 0.308                                                                   & 0.332                                                                 & 0.348                                & \textbf{0.441}                     \\ \hline
MySQL Forum       & F1-score               & 0.004        & 0.07             & 0.05           & 0.269                                                                   & 0.253                                                                 & 0.382                                & \textbf{0.449}                     \\ \hline
PG SO             & F1-score               & 0.006        & 0.201            & 0.339          & 0.299                                                                   & 0.390                                                                 & 0.321                                & \textbf{0.398}                     \\ \hline \hline
MySQL Run         & SuccessRate         & -            & 0.490            & 0.471          & 0.510                                                                   & 0.569                                                                 & \textbf{0.765}                                & 0.706                     \\ \hline
\end{tabular}
}
%\vspace{-1em}
\end{table*}
